Occlusion-Aware Search for Object Retrieval in Clutter

We address the manipulation task of retrieving a target object from a cluttered shelf. When the target object is hidden, the robot must search through the clutter for retrieving it. Solving this task requires reasoning over the likely locations of the target object. It also requires physics reasoning over multi-object interactions and future occlusions. In this work, we present a data-driven hybrid planner for generating occlusion-aware actions in closed-loop. The hybrid planner explores likely locations of the occluded target object as predicted by a learned distribution from the observation stream. The search is guided by a heuristic trained with reinforcement learning to act on observations with occlusions. We evaluate our approach in different simulation and real-world settings (video available on https://youtu.be/dY7YQ3LUVQg). The results validate that our approach can search and retrieve a target object in near real time in the real world while only being trained in simulation.

==> 8-Real-3DSim.tex <==
\section{Realistic Experiments} \label{sec:3D}
The simulation results show that the hybrid planner can be reliably used in environments with 
different physics parameters.
To further validate this finding, we test our approach in a realistic setup.
We use the 3D MuJoCo physics engine with the Deepmind Control Suite \cite{tassa2020dmcontrol}
as the execution environment, and Box2D as the simulation environment for the hybrid planner.
% The camera in mounted om the gripped with $25^0$ tilt angle.

To replicate a conservative performance of real-world object detection tools 
from a single image in clutter \cite{wang2019densefusion, xiang2017posecnn},
% (\eg, AR-markers, PoseCNN \cite{xiang2017posecnn}, DenseFusion \cite{wang2019densefusion}, etc.),
the execution environment (having access to the ground truth) would only report 
to the simulation environment 
the poses and types of objects whose more than $50\%$ of their body 
is visible within the current camera view.
% Object detection is outside the scope of this work.
% It is a well studied field and $50\%$ could be considered a conservative estimate.
% Object detection in a single image
% is already a very well studied problem
% Otherwise, an object is considered 
% we consider an object detectable in the execution environment if more than $50\%$ of its body is visible,
% \ie, the simulation environment only received the poses and types of currently detectable objects in the execution environment.

We use $m$=$4$ and $h$=$4$ as they offer a reasonable balance 
between success rate and execution time.
The shelf dimensions are W:$50$$\times$D:$35$$\times$H:$30 \ cm$.
We conduct 30
tasks with random number of obstacles, up to 10.
% 20 randomly sampled low (4 objects) and highly (9 objects) cluttered scenes. 
We also experiment with the stochastic policy 
as it showed the second best success rate in the previous experiments.
% For each task, we use the hybrid policy and the stochastic policy. 
% Experimental results are in Table~\ref{table:real_world_results_table}. 

The hybrid planner and the stochastic policy achieve a success rate of $88\%$ and $79\%$, respectively.
These results are similar to the previous experiment with high noise levels.
% We performed experiments under different clutter densities.
% Snapshots of the resulting behaviour are shown in Fig.\ref{fig:seq1} and Fig.\ref{}.
Examples of tasks solved with the hybrid planner are shown in Fig.~\ref{fig:seq1}, Fig.~\ref{fig:snapshots}, and in the attached video. 
% A video showing the performance  is available in the supplementary material.
The hybrid planner demonstrates that 
% it can control the robot for searching 
% and retrieving the target object. 
when the target object is not visible, 
the robot 
performs information-gathering actions by advancing into the shelf 
and manipulating obstacles to increase visibility.
% intentionally advances into the shelf while pushing
% the clutter around. 
% exhibiting an interactive search behaviour.
When the robot loses sight of a previously detected target object,
due for example to an obstacle blocking the camera view,
the robot focuses its search 
on the area where the target object was last seen.  
% The robot is shown to recover from situations where an obstacle
% falls within the gripper fingers.
% Furthermore, once the target object is grasped, 
% the robot manoeuvres its way backwards while avoiding 
% pushing obstacles off the shelf. 
% The robot's behaviour shows that the
% NN 
% heuristic that is driving the planner 
% stores relevant knowledge on past
% observed objects. 
% which are not anymore detected.

% In this work, ``realistic'' refers to a 3D physics simulator, Mujoco \cite{mujoco} used 
% with the Deepmind Control Suite \cite{tassa2020dmcontrol}.
% 3D physics simulator which is designed to
% mimic the real-world.
% The location of robot base is empirically optimised to minimize the robot body colliding with the shelf. 

% \begin{figure}[h]
%   \begin{center}
%   \includegraphics[width=1.0\textwidth]{figures/seq10.pdf}
%   \end{center}

% \end{figure}

%   \centering
%   \begin{subfigure}{.3\linewidth}
    % \includegraphics[width=1.0\textwidth]{figures/seq12.pdf}
%   \end{subfigure}
    % \hfill
%   \begin{subfigure}
    % \includegraphics[width=1.0\textwidth]{figures/seq10.pdf}
%   \end{subfigure}
%   \caption{Snapshots of the hybrid planner retrieving the green object.}



==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/0-Abstract.tex <==
\begin{abstract}
We address the manipulation task of retrieving a target object from a cluttered shelf.
When the target object is hidden, the robot must search through the clutter for retrieving it.
Solving this task requires reasoning over the likely locations of the target object.
It also requires physics reasoning over multi-object interactions and future occlusions.
In this work, we present a data-driven hybrid planner
for generating occlusion-aware actions in closed-loop.
The hybrid planner explores likely locations of the occluded target object
as predicted by a learned distribution from the observation stream.
The search is guided by a heuristic trained with reinforcement learning to act on observations with occlusions.
We evaluate our approach in different simulation and
real-world settings (video available on \textcolor{myblue}{https://youtu.be/dY7YQ3LUVQg}). 
The results validate that our approach can search and retrieve a target object in near real time in the real world while only being trained in simulation.
\end{abstract}


% We address the manipulation task of retrieving a target object from a cluttered shelf. When the target object is hidden, the robot must search through the clutter for retrieving it. Solving this task requires reasoning over the likely locations of the target object. It also requires physics reasoning over multi-object interactions and future occlusions. In this work, we present a data-driven hybrid planner for generating occlusion-aware actions in closed-loop. The hybrid planner explores likely locations of the occluded target object as predicted by a learned distribution from the observation stream. The search is guided by a heuristic trained with reinforcement learning to act on observations with occlusions. We evaluate our approach in different simulation and real-world settings (video available on https://youtu.be/dY7YQ3LUVQg). The results validate that our approach can search and retrieve a target object in near real time in the real world while only being trained in simulation.

% in the occluded spaces. 
% prehensile and non-prehensile 
% In this work, we present a learning approach for
% a heuristic-based hybrid planner that acts on a history of occluded observations 
% to generate prehensile and non-prehensile actions in closed-loop.

% It often involves performing an interactive search for retrieving a hidden target object.
% We propose learning occlusion-aware manipulation skills
% that can scale to environments with arbitrary number of obstacles.
% skills for exploring and evaluating action 
% a physics-based look-ahead search over a 
% learned distribution 
% We propose learning an occlusion-aware behaviour that can scale to environments with different cluuter densities
% heuristic for guiding guiding physics searched over a
% learned distribution of the location of the taget object 
% The robot can come into contact with multiple obstacles that might be hiding the target object or
% blocking access to it. 
% Solving this task necessitate sequential physics-based reasoning over occluded spaces.
% The robot must have a reactive behaviour that generalize to different 
% clutter densities as, because of occlusion, the number and shape of the hidden cannot be known a priori.
% We propose a hybrid approach that combines a learned behaviour for action generation and 
% physics-based look-ahead pllaner

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/1-Introduction.tex <==
\section{Introduction} \label{sec:INTRO}
%% -- Example -- %%
Autonomously
manipulating everyday objects 
in cluttered environments with occlusions has
% with clutter and occlusions has 
long been a target milestone in robotics research \cite{roadmap2020, christensen2016roadmap}.
As an example scenario consider Fig.~\ref{fig:seq1}, in which  the robot is tasked with retrieving 
the oil bottle from a kitchen cabinet of limited height.
The cabinet shelf is cluttered with with jars, cereal boxes, and other bottles
while the oil bottle is nowhere to be seen. 
The robot needs to push through the clutter 
to search for the oil bottle, and then reach, grasp, and pull it out
without dropping any of the other objects off the 
shelf.


%% -- Uncertainty -- %%
A sequence of prehensile and non-prehensile actions 
in a partially observable and contact-rich environment requires 
reasoning on occlusions and physics-based uncertainty. 
Even when high-accuracy object detection systems are available,
occlusion remains an inherent source of uncertainty hindering the 
search for the target object \cite{kaelbling2013integrated}.
The robot has to reason over a history of partial observations to efficiently
explore where the target object might be.
Furthermore, it is notoriously hard to predict the outcome of 
an action in multi-contact physics environments 
\cite{ronnau2013evaluation, chung2016predictable, leidner2018cognition, papallas2020non}.
Modelling error on the physics parameters such as friction, inertia, and objects shapes 
impede open-loop execution of long action sequences.

\begin{figure*}
\centering
\includegraphics[max width=1.0\textwidth]{figures/real_seq_oil_aug.pdf}
\caption{The robot is tasked with retrieving the oil bottle. The real-world images are from a gripper-mounted RGB camera. The images on the top-right are rendered from the current state of the physics simulator as recreated based on the current real-world image. The images from the simulator are used by our approach to hypothesize potential poses for the target object.
% which will then be explored by a heuristic-guided RHP.
}
\label{fig:seq1}
% \vspace{-15pt}
\end{figure*}



%% -- model-based -- %%
Most research efforts on sequential-decision making
in clutter and under partial observability 
have focused on model-based approaches. 
When the task is modelled as a
Partially Observable Markov Decision Process (POMDP)~\cite{kaelbling1998planning},
planning takes place in belief space,
that is, on a probability distribution over the actual state.
The belief is continuously updated after every interaction with the environment~\cite{li2016act, xiao2019online, pajarinen2017robotic}.
In multi-contact multi-object tasks, however, 
the physics can quickly degenerate to multi-modal 
and non-smooth distributions~\cite{agboh2020parareal}.
Hence, scaling the belief update over occluded spaces and the belief planner to
long action sequences become impractical.
%% -- model-free -- %%
Alternatively, model-free approaches with function approximators
bypass the need for a closed-form representation 
of the belief update and environment dynamics.
By directly mapping observation history to manipulation actions,
they can scale to arbitrary large state spaces and with long observation history
\cite{garg2019learning, heess2015memory, danielczuk2019mechanical}.
Sequential reasoning over future occlusions and multi-contact physics remains an open challenge
for model-free approaches.


To solve the problem of multi-object manipulation under physics uncertainty, 
heuristic-guided Receding Horizon Planning, RHP, can be used. 
RHP interleaves quick short horizon planning cycles with execution, similar 
to model predictive control.
By continuously updating the simulator state, where planning takes place, 
from real-world observations, RHP circumvents the problem of compounding modelling errors over long sequences of actions.
% diverging physics predictions that accumulates over long sequence of actions between the two environments.}
Under the assumption of a fully observable environment, 
we have shown in our previous work how RHP can be used with
a heuristic
to guide physics-based roll-outs and to estimate the cost-to-go from 
the horizon to the goal \cite{bejjani2018planning}.
This approach balances the advantages of model-based sequential reasoning 
with a model-free scalable heuristic 
\cite{bejjani2019learning, bejjani2021learning}.
% \colorbox{yellow}{highlight}
However, in a partially observable environment,
the target object is not always detected and hence cannot be simulated by RHP.
In this work, we explore learning to predict the location of 
the target object.



% To extend the advantages of RHP to partially observable environments,
% the heuristic must 
% exploit
% information from past observations.
% \add{
% We approach the search and retrieve problem 
% by leveraging 
% past observations using 
% a learned model-free heuristic with recurrent structure 
% to 
% guide a model-based look-ahead search.}
% under partial observability.}
We propose 
(\emph{i}) a data-driven approach for maintaining a distribution
over the target object's pose from a stream of partial observations
\ii and an occlusion-aware heuristic 
% for RHP to reason over the physics under partial observability. 
to run RHP under partial observability.
These two key ideas form a hybrid planner which uses the distribution to suggest 
potential target object poses
for RHP to explore.
We also present the learning architecture for simultaneously learning a generative model 
of the target object pose distribution and an occlusion-aware heuristic in a continuous action space.
We evaluate the proposed approach in environments 
with varying clutter densities, configurations, and object shapes. 
We also validate its performance in retrieving 
different target objects in the real world.
A holistic analysis of these contributions can be found in \cite{bejjani2021phd}.

% \section{Assumptions} \label{sec:ASSUM}
This work adopts the following assumptions.
A library of object type-shape pairs is given.
Objects have a uniform horizontal cross-section along the z-axis, 
and they are small enough 
to be graspable from at least one approach angle. 
They are placed on the same horizontal 
surface.
% within the shelf space.
The robot's actions are pose increments
parallel to the manipulation surface 
in the planar Cartesian space of the gripper.
We do not consider 
access to a separate storage space.

% ######################################################
% ######################################################
% ######################################################
% ######################################################
% simulation and in the real world different with varying clutter densities and configurations.

% The state of the execution environment (\eg, real-world) is mapped to
% the simulation environment where RHP is performed. 
% The returned action by RHP is then executed in the execution environment.

% Online POMDP planners 
% have achieved impressive results in manipulation tasks 
% where explicit modelling of uncertainty is tractable 
% \cite{li2016act, xiao2019online, pajarinen2017robotic}. 
% In partially observable environments, they have successfully 
% demonstrated reactive behaviours on 
% single object manipulation tasks \cite{garg2019learning, heess2015memory, danielczuk2019mechanical}.

%For instance, acting on a hidden space may push unseen objects off  the shelf or cause the target object to become wedged into a corner.
% , adding to the future-state uncertainty.
%Depending on the exact physics parameters such as friction and inertia, the same pushing action can  lead to very different reaction chains.
%%MATTEO: I commented some stuff because it felt like we were rambling on too much.


% a single state in a physics simulator where planning is performed. 
% RHP is queried over the simulator state. 
% By running RHP in closed-loop, compounding errors between the 
% execution environment and the planning environment remains bounded. 
% RHP alternates between real-world execution and physics-based look-ahead planning in simulation. 
% for real-time applications \cite{lowrey2018plan}.
% combines the sequential reasoning 
% offered by model-based methods
% with the scalability of model-free methods \cite{lowrey2018plan}. 
% , in a discrete action space,

% , each with different likely target object pose,

% efficiently maintain relevant 
% while also accounting for the physics and information gathering
% consequence of an action n
% account for 
% object interactions that might take place outside the sensor FOV while the robot is moving. Also, maintaining information on previously searched spaces and detected objects are essential for efficiently finding and retrieving a desired object.
% To extend the advantages of RHP to partially observable environment,

% We present a framework for running the hybrid planner in closed-loop, 
% alternating between the execution environment and planning environment.
%  A


% • A learning process for simultaneously learning a generative model for reconstructing probable states and a
% heuristic for RHP.
% • An occlusion-aware heuristic that reasons over a history
% of partial observations to guide RHP in a continuous
% action space.
% • A hybrid planner for running and evaluating RHP
% queries over partially observable states.
% • A colour-labelled image for representing occluded environments.
% We evaluate the proposed approach in different simulation
% environments with varying clutter densities and artificially
% injected noise.



% This paper extends RHP to reason over occlusions 
% for real time search and retrieve manipulation tasks.

% We present 

% a data driven approach for learning a heuristic that can simultaneously 
% estimate like poses of the target object and act as a heuristic for RHP.


% In this paper, we attempt to answer the questions of 
% \i how to maintain a distribution over likely poses of the target object 
% without explicitly modelling a belief over a large and continuous state space,
% \ii how to learn an occlusion-aware heuristic for a physics-based RHP to reason over a history of partial observations,
% and \iii how to represent partial observations and task priors while ensuring generalization
% over different clutter densities and object shapes.

% Extending the advantages of RHP to partially observable environments remains under-explored.




% We present an approach for searching and retrieving a target object from a cluttered environment with occlusions.

% We present a framework built around a novel hybrid planner
% for searching and retrieving a target object from a cluttered environment with occlusions.
% In a closed-loop control cycle, the framework provides the hybrid planner with 2D abstract representation
% of the current observation 
% The framework combines partial observations from the execution environment with task invariant information, \eg shelf walls, location of the shelf edge, etc.) 
% to generate an 2D abstract representation of   
% The hybrid planner is based on a model-free learned heuristic that action on the
% observation ste


%% -- Our solution -- %%
% To tackle the physics-based retrieving tasks, 
% We present a framework around a novel hybrid policy 
% for searching and retrieving a target object,  
% in real-time, from a cluttered environment with occlusions.
% The proposed
% % We present a hybrid approach 
% that combines the sequential reasoning offered by model-based methods
% with the scalability of model-free methods. 
% By providing a model-based RHP with an occlusion-aware heuristic, 
% RHP can explore partially observable states in real-time.
% As the target object is not always detected in the environment, and hence cannot be simulated in physics roll-outs, we train a model-free generative method to 
% estimate likely locations of the target object 
% based on the observation history.
% These locations are used to reconstruct potential
% root states to be explored by RHP.

% The contributions of this paper can be stated as follows:
% \begin{itemize}
%     \item A learning process for simultaneously learning
%         a generative model for reconstructing probable states and a heuristic for RHP.
%     \item \add{An occlusion-aware heuristic that reasons over a history of partial observations to guide RHP in a continuous action space.}
%     \item A hybrid planner for running and evaluating RHP queries over partially observable states.
%     \item \add{A colour-labelled image for representing occluded environments.}
% \end{itemize}
% We evaluate the proposed approach in different simulation environments
% and real-world shelf environments 
% with varying clutter densities and artificially injected noise.



% such domains become inefficient.

% \add{Alternatively, shortening the planned action sequence, 
% using Receding Horizon Planning, RHP,
% have proven particularly useful in reducing physics-based uncertainty
% \cite{bejjani2018planning,bejjani2019learning}.
% RHP relies on using a heuristic to efficiently explore 
% and evaluate roll-outs up-to a short 
% horizon from a single root state \cite{lowrey2018plan},
% then estimating the cost-to-go the horizon to the goal.
% However, they remain under-explored in partially observable environments.}

% Alternative model-based approaches rely on planning 
% over black-box physics simulators. 
% Although the dynamics can only be reliably 
% approximated for a few steps into the future, 
% conditional planning and online planning 
% are capable of leveraging these models to 
% reduce physics and pose uncertainties in high-dimensional spaces
% \cite{leidner2018cognition, king2017unobservable}.
% For real-time applications,
% heuristic-guided Receding Horizon Planning, RHP, has proven to be 
% a robust tool for physics-based planning \cite{bejjani2018planning,bejjani2019learning}.
% RHP relies on its heuristic to efficiently explore 
% and evaluate a small number of roll-outs up-to a short 
% horizon from a single root state \cite{lowrey2018plan}.
% However, they remain under-explored in cluttered 
% environments with occlusions.
% Emerging model-free approaches with function approximation
% as viable methods for reactive and 
% generalizable behaviour have fostered interest
% in their deployment in partially observable environments 
% \cite{hausknecht2015deep, igl2018deep}.
% are based on a direct mapping 
% from observation history to manipulation actions.
% Function approximators, with appropriate inductive biases in their structures,
% bypass the need for a closed-form representation 
% of the belief update and environment dynamics.
% tasks that 
% do not require significant long-term reasoning over the physics, such as 

% \commentl{it's not really real world.}
% To the best of our knowledge, the proposed approach is the first that can consistently retrieve a desired object in real-time from a partially observable and cluttered shelf 
% without employing pick-and-place decluttering procedures. 


% In addition, we propose learning a model-free heuristic that 
% will enable the RHP to 
% reason over occluded representations of these states.

% we propose a model-free generative method for 
% reconstructing potential states to explored by 
% RHP while under partial observably.
% As a state is not always fully manifested for RHP to explore,
% As the target object is not always detectable 
% and hence cannot be simulated for RHP exploration,
% we propose a model-free generative method for 
% reconstructing states with potential to explored by 
% RHP while under partial observably.
% reconstructing potential states to explored by 
% RHP while under partial observably.
% in an observation, \eg, the target object is not detected,

% They remain mostly suited for tasks where actions 
% are only constrained by finding a collision-free paths 
% to manipulate an object \cite{pajarinen2017robotic}.



% However, as multi-contact physics can quickly degenerate to 
% multimodal and non-smooth distributions,
% efficiently scaling the belief update to  
% high-dimensional spaces with unknown number of occluded objects is not straightforward.

% Online POMDP solvers remain mostly suitable for tasks where actions 
% are only constrained by finding a collision-free paths 
% to manipulate an object
% \cite{pajarinen2017robotic}.


% propose hybrid approach that uses both model-free and model-based to run RHP
% over 
% learning a model-free heuristic that will enable the model-based RHP to reason over the physics under occlusion.
% we propose a hybrid approach that uses both model-free and model-based methods for solving fetching tasks.
% We propose learning a model-free heuristic that will enable the model-based RHP to reason over occlusion.
% We a
% In this paper, we propose a hybrid approach that uses both model-free and model-based methods for solving, in real-time, fetching tasks.
% To tackle physics-based fetching tasks, this work focuses on have adapting RHP  
% in environments  
% rich with multi-object contacts and occlusion. 

% \i A model-free approach for generating estimates of the
% actual state.
% \ii A model-free heuristic for accelerating a model-based 
% Receding Horizon Planning, RHP, and for evaluating the long-term impact of potential actions on the estimated states.

% We explore the potential of these approaches in manipulation tasks that require long-term reasoning over the physics with occlusion in the environment.

% For example, convolutional NNs can capture spatial properties for generalization 
% over a large and continuous observation space, such as random number and shapes of objects, 
% while recurrent NNs can exploit the sequential nature of 
% the observations to maintain relevant past information \cite{karkus2017qmdp}.


% the physics in multi-contact environments quickly unfold to 
% multimodal and non-smooth distributions over future states

% representing and updating the belief 
% in high-dimensional environments, particularly with unknown number of occluded objects,
% and cantact physics that can quickly unfold to 
% multimodal and non-smooth distributions over future states

% make the application of online POMDP solvers less straightforward.

% But, 
% as the physics in multi-contact environments quickly unfold to 
% multimodal and non-smooth distributions over future states \cite{agboh2019parareal},

% as scaling these approaches to high-dimensional environments with unknown number of occluded objects
% and cantact physics that can quickly unfold to 
% multimodal and non-smooth distributions over future states

% as scaling these approaches to high-dimensional environments with unknown number of occluded objects
% and contact multi contact physics that can quickly unfold to 
% multimodal and non-smooth distributions over future states \cite{agboh2019parareal},

% as the physics in multi-contact environments quickly unfold to 
% multimodal and non-smooth distributions over future states \cite{agboh2019parareal},

% scaling these approaches to high-dimensional environments with unknown number of occluded objects
% make the application of POMDP solvers less straightforward

% They mostly suited manipulation tasks where the actions 
% are only constrained by finding a collision-free paths 
% to grasp or push an object
% \cite{pajarinen2017robotic}.

% Our approach interleaves real-world execution with model-based heuristic-guided Receding Horizon Planning (RHP).
% The hybrid approach consist of look-ahead planning on learned estimates of the
% underlying state. 
% The observation from the real world is mapped to a compact image-based representation.
% In simulation, RHP is rooted at learned estimates of the underlying state while 
% its search is guided by a learned heuristic acting on the observation history.
% \i A colour-labelled image-based representation of the observation space which combines current sensory data with task priors for greater generalization.
% \ii A model-free model-based hybrid approach for action generation in partially observable environments complex dynamics.
% \iii Simulation and real-world demonstrations assessing the performance of our proposed approach compared to similar existing work.
%% \\ Our solution \\ %%

% The physics in cluttered environment often unfold to 
% multimodal and non-smooth distributions over future states \cite{agboh2019parareal}.

% - model-free policy - %
% Learning-based model-free approaches have been proven to produce a reactive behaviour 
% that scales to large and continuous state and action spaces.
% They are mostly studied in applications where future and current state uncertainties are addressed independently \cite{viereck2017learning} \cite{Wirnshofer2020controlling}. 
% Leveraging model-free approaches to account for these two types 
% of uncertainties simultaneously remains largely unexplored. 
%% \\ Future and Current state uncertainty \\ %%

% They often rely on planning in the belief space, a proxy that summarizes the
% observation history.  
% State-of-the-art online POMDP planners use
% a state estimator (Bayesian filter, Kalman filter, etc.) 
% to maintain a probability distribution over the actual state. 
% An online planer is then used to map belief states to actions \cite{li2016act, xiao2019online}.

% the 
% modelling of the problem have been
% use to plan on a belief space that captures past information 
% such as previously searched spaces and observed objects \cite{}. 
% when action generation must also be conditioned by the observation history,
% such as previously searched spaces and observed objects \cite{bohg2017interactive}. 

% More recently, Partially Observable Markov Decision Process, POMDP, planners have become scalable to reasonably long observation history and large observation space mitigating the curse of history and dimensional \cite{somani2013despot, bohg2017interactive}.
% Albeit, maintaining real-time operation requires 

% operating in real-time remains limited to operating on a set of discrete actions where explicit probability distribution over the effect of an action can be maintained. 

% are one way to leverage available physics simulators 
% to address the uncertainties and adapt accordingly in 
% environments with non-linear and complex dynamics.

% State-of-the-art online POMDP planners can now scale to reasonably long horizon and 
% large observation space 
% mitigating the curse of history and dimensionality \cite{somani2013despot}. 

% They rely on planning in the belief space rather than the actual state space.  
% Using a state estimator (Bayesian filter, Kalman filter, etc.), a probability distribution is generated over the underlying state space of the domain. 
% A controller, often planning in a deterministic approximation of the model, 
% is then used to map belief states to actions.

% Keep track of previouslt

% Planning under current state uncertainty is often modelled as a Partially Observable Markov Decision Process, POMDP,
% which relies on planning in the belief space rather than the actual state space.  
% Using a state estimator (Bayesian filter, Kalman filter, etc.), a probability distribution is generated 
% over the underlying state space of the domain. 
% A controller, often planning in a deterministic approximation of the model, 
% is then used to map belief states to actions.
% State-of-the-art online POMDP can scale to reasonably long horizon and 
% large observation space mitigating the curse of history and dimensional \cite{somani2013despot, bohg2017interactive}. 
% Albeit, operating in real-time remains limited to operating on a set of discrete actions where explicit probability distribution over the effect of an action can be maintained. 




% The physics evolve along non-linear and complex dynamics leading to 
% multimodal and non-smooth distributions over future states \cite{agboh2019parareal}.

% This makes methods that rely on a predefined number of objects 
% for manipulation under uncertainty inapplicable 
% \cite{king2017unobservable, li2016act}. 

% Conditional planning and online planning \cite{dogar2012planning, leidner2018cognition} are one way to address unexpected deviations from the plan.

% Due to the cost associated with rolling out the physics, it remains challenging 
% to scale these approaches for solving long-horizon sequential decision-making problems
% whilst maintaining a real-time reactive behaviour. 

% For example, the same pushing action of an object 
% with the fingertip of the gripper can 
% lead to very different results.
% The object might fall in or outside the gripper fingers 
% depending on the underlying physics parameters, 
% such as friction and inertia, and the actual state, such as if 
% there is hidden obstacle acting on the object.

% The vast majority of research on manipulation in clutter under uncertainty have 
% adopted a model-based approach whether as a POMDP planning, conditional, uncertainty reducing ...

% In this work we consider the following question: How
% do we generalize this analysis to create robust open-loop
% pushing trajectories for use in rearrangement tasks?
% we aim to achieve level of manipulation skills where the robot
% if the salt shaker is hidden right behind an obstacle that the robot is 
% trying to push out of its way or if the friction cone between the robot and the obstacle is not accurately modelled, the obstacle might either push the salt shaker further away from the robot or fall into the robot's grasp obstructing it motion. 


% Available physics simulator can only reliably 
% approximate very few step intro the future.
% the distribution over future states in a 
% multi-contact physics environment is notorious hard even 
% with fully observable current state.
% The environment evolve along non-linear and complex dynamics
% which leads to multimodal and non-smooth distributions.
% Available physics simulator can only approximate how the 
% environment will 
% This means that the same action can produce
% very different effects depending on how it is executed

% current between robot and objects causes physics
% to evolve in complex, non-linear ways and quickly leads
% to multimodal and non-smooth distributions. This makes
% methods that rely on closed form representation of the
% stochastic dynamics inapplicable


% the robot to reason over future and current state uncertainties.
% and with not enough shelf space for collision-free decluttering actions,
% Often, top-down pick and place operations for decluttering the cabinet 
% are not feasible due to narrow shelf heights and other shelves being 
% already packed \cite{correll2016analysis, eppner2016lessons}. 
% Instead, fetching the salt shaker





% The robot is left with having to interact and navigate its way through the clutter 
% to search, reach, grasp, and pull-out the cup while 
% avoiding to drop of any of the movable obstacles off the shelf. 
% Acting in physics rich and partially observable environments requires 
% the robot to reason over future and current state uncertainties.
%% \\ Example and context \\ %%

%% -- Future and Current state uncertainty -- %%
% - Future - %
% The uncertainty associated with the future outcome of an action or a sequence of actions 
% arises from the inaccuracies in modelling how the physics of the environment will unfold.
% Model-based approaches, such as conditional planning and online planning \cite{dogar2012planning, leidner2018cognition}, are one way to address unexpected deviations from the plan.
% Due to the cost associated with rolling out the physics, it remains challenging 
% to scale these approaches for solving long-horizon sequential decision-making problems
% whilst maintaining a real-time reactive behaviour. 

% - Current - %
% Current state uncertainty is unavoidable in many real-world applications due to occlusion
% by clutter even when high accuracy localization and detection systems are available.
% Planning under current state uncertainty is often modelled as a Partially Observable Markov Decision Process, POMDP,
% which relies on planning in the belief space rather than the actual state space.  
% Using a state estimator (Bayesian filter, Kalman filter, etc.), a probability distribution is generated 
% over the underlying state space of the domain. 
% A controller, often planning in a deterministic approximation of the model, 
% is then used to map belief states to actions.
% State-of-the-art online POMDP can scale to reasonably long horizon and 
% large observation space mitigating the curse of history and dimensional \cite{somani2013despot, bohg2017interactive}. 
% Albeit, operating in real-time remains limited to operating on a set of discrete actions where explicit probability distribution over the effect of an action can be maintained. 

% - model-free policy - %
% Learning-based model-free approaches have been proven to produce a reactive behaviour 
% that scales to large and continuous state and action spaces.
% They are mostly studied in applications where future and current state uncertainties are addressed independently \cite{viereck2017learning} \cite{Wirnshofer2020controlling}. 
% Leveraging model-free approaches to account for these two types 
% of uncertainties simultaneously remains largely unexplored. 
%% \\ Future and Current state uncertainty \\ %%






%% -- Scratch -- %%
% To the best our knowledge this is the first work to achieve model-free continuous control for physics-based manipulation in partially observable and cluttered environments. 
% Two action generation strategies. A model-free stochastic policy approach,  
% and a model-based and model-free hybrid for environment complex dynamics.
% receding horizon manipulation planning
% An investigation on the potential use of a model-based and model-free hybrid for receding horizon manipulation planning.
% \ii A recurrent neural model that embeds image-based observations' history 
% for conditioning continuous control actions generation. 
%% -- search and manipulate -- %%
% Multi-object manipulation in cluttered and partially observable environments 
% often requires a synergy between a search and a retrieve behaviour (cite). 
% When uncertainty over the current belief state is too high for the desired object 
% to be safely retrieved, a sequence of information gathering actions a performed. 
% For instance, an obstructing object can be moved to the side to clear the camera view \cite{li2016act}, 
% or the camera can be moved around to capture the environment from different perspectives \cite{kaelbling2013integrated}. 
% An underlying assumption for treating a search and a retrieve behaviour independently is that 
% information gathering mostly sharpens the probability distribution of the belief space.
% However, in contexts where multiple objects can interact with one another, trying to uncover one part of 
% the state space can lead to a loss of information over previously perceived parts. 
% Moving the robot in tight spaces, whether during a search or a retrieve behaviour, can cause 
% an oblivious (hard to predict) chain of object-to-object and robot-to-object interactions. 
% Unless the decision-making process jointly considers the search and the retrieve behaviour, the robot 
% can potentially fall into alternating between these two behaviours, resulting in more 
% planning and execution operations than necessary to solve the task. 
%% \\ search and manipulate \\ %%
% In this paper, we propose learning a model-free policy for solving manipulation tasks under current and future state uncertainties while avoiding any explicit distinction between high-level search and retrieve actions. 
%% \\ Scratch \\ %%


==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/2-RelatedWork.tex <==
\section{Related Work} \label{sec:SOTA}
%% -- Model-based -- %%
\emph{\textbf{POMDP planners:}} In the presence of occlusions, manipulation in clutter 
is often associated with active search, that is,
leveraging manipulation actions to simultaneously 
gain visibility and accessibility \cite{bohg2017interactive}.
Thanks to recent advances in model-based online planners under uncertainty \cite{somani2013despot, xiao2019online, papallas2020online, bejjani2015automated}, 
% like DESPOT \cite{somani2013despot} and PA-POMCP \cite{xiao2019online}, 
this field is gaining momentum towards achieving everyday 
% real-world 
manipulation tasks.
% Li \etal \cite{li2016act} address uncertainty on the object 
% type that is caused by partial occlusion. 
% They propose exploiting spatial constraints to reduce the number of feasible 
% actions to be explored.
% by a fixed-length horizon planner. 
% Hence, they can decide online on which object to be moved to minimize occlusion. 
% In addition to spatial constraints, 
Wong \etal \cite{wong2013manipulation} 
use object semantics and spatial constraints to focus the search in shelves where the clutter is
most similar to the target object.
% They minimize the number of active search operations by favouring the search of occluded 
% spaces where the semantics of observed objects are most similar to the target object.  
Pajarinen \etal \cite{pajarinen2017robotic} solve long-horizon multi-object 
manipulation by combining particle filtering  
and value estimates in an online POMDP solver.
These approaches 
% stated so far 
have largely overcome the computational 
complexity 
associated with 
large state space and observation history. 
However, they avoid multi-object contacts by 
planning with collision-free actions. 
% involving single objects. 
This constraint reduces planning time, but it also prevents 
the robot from exploiting the full dynamics of the domain.

% Multiple studies have proven that multi-object 
% manipulation with physics-based
% actions, such as pushing, 
% are particularly useful when there is no collision-free 
% path to reach an object
% \cite{papallas2020online, agboh2018real}.
% King \etal \cite{king2017unobservable} propose a pushing-based
% online planner in cluttered environments which 
% accounts for uncertainty on the objects' poses.
% Dogar \etal \cite{dogar2014object} use a heuristic to 
% plan pushing actions for object search under occlusion.
% In this work, we do not make an explicit distinction between 
% prehensile and non-prehensile actions.
% Instead, the robot's motion is controlled over a continuous action space.
%% \\ Model-based \\ %%

%% -- Model-free -- %%
\emph{\textbf{Model-free policies with recurrent units:}} 
Model-free policies are at the core of many applications that 
necessitate reactive decision-making under uncertainty.
Heess \etal \cite{heess2015memory} show that by using 
Long Short-Term Memory (LSTM) cells as a tool to summarize 
a history of partial observations, 
% instead of conditioning the policy on the entire history, 
it is possible to train a policy for pushing an object to an initially observed pose. 
Karkus \etal \cite{karkus2017qmdp} propose a model-free approach that trains a neural network (NN)
on expert demonstrations to approximate a Bayesian filter and a POMDP planner.
% Garg \etal \cite{garg2019learning} 
% show that by representing the policy with a NN with recurrent layers, the policy can 
% integrate noisy observations to generate grasp actions.
%These approaches demonstrate the potential of model-free policies with recurrent units to reason over a history of partial observations.
% while aslo generalize over a
% large and continuous observation space.
These approaches are focused on single object manipulation and do not ensure
long-term reasoning over the physics.
%% \\ Model-free \\ %%

\emph{\textbf{Searching in clutter through manipulation:}}
The goal of our work is most aligned with the objective of
Danielczuk~\etal~\cite{danielczuk2019mechanical}. 
They define it as
``Mechanical Search'', a long sequence of actions for 
retrieving a target object from a cluttered environment 
within a fixed task horizon while minimizing time.
They propose a data-driven framework for detecting then performing 
either push, suction, or grasp actions until the target 
object is found.
They tackle top-down bin decluttering by removing obstructing objects
until the target is reachable.
Such an approach requires a separate storage space to hold obstructing objects. 
To address environments where a separate storage space is not available,  
Gupta~\etal~\cite{gupta2013interactive} 
and Dogar~\etal~\cite{dogar2014object}
% interleaves look-ahead planning
interleaves planning
with object manipulation on a shelf.
They both propose moving objects to unoccupied spaces within the same shelf
to increase 
scene visibility from a fixed camera view angle.
% In a similar shelf setup,
% Dogar \etal \cite{dogar2014object} use a heuristic to 
% plan pushing actions until the target object is found.
The approaches stated so far perform the search by
% The methods stated so far
% approach the problem of searching in clutter by 
manipulating one object at a time, 
avoiding sequential reasoning over multi-contact physics.
Avoiding 
all obstacles 
remains, however, impossible (and often undesirable) in many 
partially observable and cluttered environments.
Most recently, Novkovic \etal \cite{novkovic2020object} propose a 
closed-loop decision making scheme for 
generating push action in a 
multi-contact physics environment
with a top-mounted camera. 
Their approach relies on encoding the observation history in 
a discretized representation of the environment. 
The encoding is used by an RL trained policy to generate 
the next push action for revealing hidden spaces. 
% The goal of our work is most aligned with the objective of \cite{danielczuk2019mechanical}, 
% but in environments reminiscent to \cite{gupta2013interactive, dogar2014object}.
% We adopt a similar decision making scheme,
% but we avoid the limitations
% of a discretized representation by relying on the NN's recurrent
% units to capture the observation history.
We adopt a similar decision making scheme,
but we avoid the limitations
of encoding the observation history in a discretized representation.
Instead, we rely on the NN's recurrent
units to capture the observation history.


% In setting where objects cannot be removed permanently from the
% scene, such as by placing them in another storage space,

% They necessitate a free space the hold obstructing object, 
% whether separate storage bins
% or unoccupied shelf space.
% as such, sequential reasoning over multi-contact physics can be avoided.
% sequential reasoning over multi-contact physics

% , and with that comes the necessity of a reactive system.

% to rearrange objects such that 

% Their objective is most reminiscent to ours.

% picking setting
% whereas we look into planar manipulation.



%% -- RHP  -- %%
% In environments where the effects of an erroneous action 
% cannot be immediately mitigated by a reactive policy,
% look-ahead planning have shown to compensate 
% for deficiencies in anticipating the effects of an action
% \cite{agboh2018pushing, bejjani2018planning}. 
% We avoid Monte-Carlo look-ahead based planners as they require simulating 
% a large number of computationally expensive physics roll-outs
% \cite{hayashi2019online, song2019multi}.
% Yet, inspired by the contribution of look-ahead planning to robustness in critical domains,
% we extend heuristic-guided RHP
% to operate in environments with occlusions.




%% -- hybrid  -- %%
% More recently, methods that combine mode-based and model-free techniques
% are showing impressive performance in handling the complex physics of an 
% object under uncertainty. 
% Hayashi \etal \cite{hayashi2019online} trains a NN to continuously update the physics parameters of a model-based pushing planner in clutter. 
% Wirnshofer \cite{wirnshofercontrolling}
%% -- hybrid -- %%
% for generating goal-oriented actions with possible extension to continuous control applications.
% Instead of directly acting on a learned policy, these approaches
% leverages existing physics models to perform heuristic-guided online planning.
% We avoid Monte-Carlo based planners, such as \cite{silver2010monte}, as
% the computation cost of simulating a relatively large 
% number of physics roll-outs up-to a terminal state
% make them inefficient for real-time applications \cite{song2019multi}.
% Yet, 
% These approaches assume a fully observable environment.
% In this work, 
% online multi-step look-ahead planning where 
% the learned policy is used as a heuristic. 

% In many applications with long horizon and/or complex environment dynamics, 
% heuristic-guided Receding Horizon Planning (RHP), have shown to compensate 
% for deficiencies of a deep learning 
% trained NN in approximating the optimal policy \cite{anthony2017thinking, bejjani2018planning, lowrey2018plan}. 
% Instead of directly acting on the learned policy, RHP exploits 
% the availability of a model to perform online multi-step look-ahead planning where 
% the learned policy is used as a heuristic. 
% We further these approaches to 
% planning in partially observable environments. 
%% \\ hybrid and RHP \\ %%


% There uses in cluttered and occluded environments remains under explored.
% 
% information and generate goal-oriented actions with possible extension to continuous control applications.
% with 
% integrated memory cells with possible extension to continuous control applications.
% For reasons, like partial observably, physics learning, or sensory noise integration, 
% recurrent neurons are becoming more prevalent in may NN-based 
% controlled robotics applications \cite{driess2020deep, garg2019learning, rahmatizadeh2018virtual}.
% In their work on bridging the sim-to-real gap with RL, 
% Peng \etal \cite{peng2017sim} use recurrent neurons, namely LSTM, 
% as part of the NN architecture to capture the physics of pushing an object on a surface.

% In this paper, we adopt a continuous action space as it offers fine 
% control over the robot's motion, but we also address action generation
% in environments with multi-object contacts.

% Autonomously manipulating objects in clutter has 
% long been a target milestone in robotics research.

% king2017unobservable}.
% Modern light weight manipulators
% can afford to deliberately come into contact with environment,
% which is  a key element for when there is no collision-free 
% trajectory to reach the desired object.
% a robotic agent to get in deliberate soft contact with their
% environment, which is a key element for many manipulation
% when there is no collision-free trajectory to reach the desired object

% This field has long been addressed with model based approaches thanks to
% Leveraging Action in
% Perception and Perception in Action

% Automated manipulation planning with a universal robotic
% agent in domestic environments has ever since been a major goal in robotics research, as well as in research on autonomous agents. Recently, this field has regained momentum thanks to affordable and safe light weight robots such
% as the LBR III [14]. These compliant manipulators enable
% a robotic agent to get in deliberate soft contact with their
% environment, which is a key element for many manipulation
% tasks, including wiping of surfac

% The advent of efficient POMDP solvers that can be used online, 
% like DESPOT \cite{somani2013despot} and PA-POMCP \cite{xiao2019online}, 
% have fostered the development of model-based approaches in multi-object 
% environments where searching for an object is not confined to a visual 
% search but also active manipulation.
% n particularly
% when there is no collision-free trajectory to reach the desired object.
%% \\ Model-based \\ %%





%% -- Scratch -- %%
% They extended their approach to operate on images. However, the image-based experiments were limited to controlling an under actuated pendulum to reach an initially observed target. 
% In many real-world setups, it not only advantageous to leverage environment contacts but 
% timetheir adopted RL training procedures is focused on single object manipulation.
% Compatible Policy Search for Manipulation and Navigation under Partial Observability
% either by discretizing the state space into an occupancy grid or by using particle filtering to reduce the sample size of planning instances. 
% and long horizon planning by a combination of particle filtering, 
% he planning is performed on the level of semantic actions and locations
% particle, weighted set of states, \cite{li2016act}
% Occupancy grid state space, discrete action spaces, container semantics \cite{wong2013manipulation}.
% Multi-object manipulation does not consider complex physics interactions,
% adapts object specific action success probabilities \cite{pajarinen2017robotic}

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/3-Methodology.tex <==
\section{Problem Definition} \label{sec:METHO}
% % \begin{figure}[b]
% \begin{wrapfigure}{r}{0.23\textwidth}
% \centering
%   \includegraphics[width=0.23\textwidth]{figures/environment3.jpg}
% %   \vspace{-10pt}
%   \caption{Environment setup.}
%   \label{fig:env}
% % \end{figure}
% \end{wrapfigure}
The robot's task is to retrieve a target object from a shelf 
of limited height
without dropping 
any of the other objects off the shelf.
The robot carries a gripper-mounted camera.
% A typical setup is shown in Fig.~\ref{fig:env}. 
We treat the search, reach, grasp, and pull-out of the target object as 
a single optimization problem with the objective of minimizing the total number of actions
for retrieving the target object.


\subsection{Formalism} \label{sec:FORM}
%% -- POMDP -- %%
We model the problem as a POMDP  $\langle S, A, O, T, \Omega, r, \gamma \rangle$, where
$S$ is the set of states, $A$ the set of continuous actions, $O$ the set of possible observations, $T : S \times A \times S     \rightarrow [0,1]$  the transition function,  $\Omega : S \times O \rightarrow [0,1]$ the observation model, 
$r:  S \times A \times S \rightarrow  \mathbb{R}$ is the reward function, and $\gamma \in [0,1)$ is the discount factor. 
% The underlying state is a vector of variables $s=\{\mathcal{R}, \mathcal{O}_1, \mathcal{O}_2, \ldots  \}$,
$s=\{Rob, Obj_1, Obj_2, \ldots  \}$,
in which 
$Rob$ is the robot's end-effector pose, shape, and gripper's state; 
% $Shelf$ describes the shape of the shelf's walls and the location of its open edge; 
$Obj_i$ describes an object's pose, shape, and type.
% , with $i=1$ being the $target$ object. 
An observation $o \in O$ contains a subset of the state variables (\eg, the visible objects), and the geometry of occluded spaces: the shadowed areas behind objects and areas outside the
camera's field of view (FOV). 
% \commentl{This isn't very clear, a description in terms of variables like for the state would be better.}

%% -- Goal -- %%
Since the state is not always accessible because of occlusions, 
decision making relies  on maintaining a belief $b : S \rightarrow [0,1]$ as a distribution over possible states.
% , which is a probability distribution over the states 
% with $b' = b'(s'|b,a,o)$ where $a\in A$, $s\in S$, and $o=$??.
% The belief is continuously updated from the observation history. 
A POMDP policy $\pi$ is a function that maps a belief $b$ to an action $a$. 
The value $V$ of a policy $\pi$ 
at belief $b_t$ at time $t$ is the expected \emph{return}:
$
V_{\pi} = \mathbb{E}_{a\sim\pi, s_t \sim b_t} [\sum_{k=t} \gamma^{k-t} r_{k+1}] 
$
% \begin{equation}\label{eq:JofPi}
% V_{\pi} = \mathbb{E}_{a\sim\pi} [\sum_{k=t} \gamma^{k-t} r_{k+1}| b]. 
% \end{equation} 
where $r_{t+1} = r(s_t,a_t, s_{t+1})$.
We avoid shaping the reward function in order not to skew the robot's behaviour towards 
any preconceived human intuition which might artificially limit the return. 
% \commentl{I don't understand what you mean here by minimum number of actions.}
Instead, we opt for a constant 
% \rm{uniform} 
negative reward of $-1$ per action. 
When an object is dropped, the task is terminated and 
an additional large negative reward of $-50$ is received.
% \rm{casting the problem as a stochastic shortest path.}
%% \\ Goal \\ %%


\subsection{Overview} \label{sec:OVER}
We use the closed-loop decision making scheme shown in Fig.\ref{fig:control},
where we observe the environment, plan, execute the first action of the plan, then loop back to the observe step.\\
% We adopt the \emph{observe-plan-act} closed-loop decision making scheme shown in Fig.~\ref{fig:control}.\\
% The observation and planning takes place in a physics simulation environment and actions in the execution environment.
\emph{\textbf{Observe}}: 
The poses and types of visible objects in the execution environment,
as detected by the gripper-mounted camera,
and task priors are used to 
recreate, in the simulation environment, a state with the currently detected objects.
The current observation,
a top-down view of the scene,
is rendered from the simulation
environment (Sec.\ref{sec:OBSER}). 
% But since the location of the
% target object is not always known, it cannot be placed in the observation. 
\\
\emph{\textbf{Plan}}:
The hybrid planner uses 
the observation history, including the current observation,
to update a distribution over the likely poses of the target object.
The estimated target object poses are used to hypothesize 
root states, each with a target object placed at one of the predicted poses.
If a predicted pose is in an occluded area, 
the target object would still be added to the physics simulator but it will be occluded in the observation.
RHP uses its occlusion-aware heuristic (a stochastic policy and its value function) 
to explore and evaluate physics roll-outs from the root states.
RHP returns the best action to execute at each root state 
and its corresponding estimated \emph{return} (Sec.\ref{sec:HYB}).\\
\emph{\textbf{Execute}}:
The \emph{returns} are weighted by the likelihood of their root states, 
and the action with the highest weighted \emph{return} 
is executed in the execution environment (Sec.\ref{sec:HYB}).
After a single step of execution, the system goes back to the observation step,
for a closed-loop execution.
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/control1.pdf}
  \caption[]{Approach overview. An example with the small jar at the back of the shelf as the target object.}
  \label{fig:control}
\end{figure}
% An example with the horseradish jar (the small white jar) being the target object.
% \begin{itemize}
%     \item Observe: 
    
%     The current observation consist of an abstract colour-laballed image that combines data from the execution environment and task priors while capturing
%     spatial information on occluded and observable spaces.
%     It is rendered from the simulation environment (Sec.\ref{sec:OBSER}).
%     \item Plan: We then run the hybrid planner in a physics 
%     simulation environment from which observations are rendered.
%     The observation history, including the current observation,
%     is used to update 
%     a distribution over the likely poses of the target object.
%     % recreate mutliple state with 
%     % The hybrid planner starts by querying a NN to estimate like poses of the target object,
%     The estimated target object poses are used to hypothesize 
%     partially observable root states for RHP.
%     RHP uses its occlusion-aware heuristic (a stochastic policy and its value function) 
%     to explore and evaluate the root states.
%     RHP returns the best action to execute at each of the root states and its corresponding \emph{return}.
%     \item Act: The \emph{returns} are weighted by the likelihood of their root states, and
%     the action with the highest weighted \emph{return} 
%     is executed in the execution environment (Sec.\ref{sec:HYB}). 
% \end{itemize}

At the core of our approach is a NN with recurrent units that maps 
an observation history into: 
(\emph{i}) a distribution over the pose of the target object $\hat{y}(\Bar{o})$ with $\Bar{o}$ being the observation history,
\ii a stochastic policy $\pi(.|\Bar{o})$, 
\iii and its corresponding value function $V_{\pi}(\Bar{o})$, 
(Sec.~\ref{sec:MOD_FREE}). 
% Prior to using the NN at execution time, 
The NN is trained in the 
physics simulation environment 
% following 
% an Imitation Learning (IL), 
% then a 
with 
curriculum-based Reinforcement Learning (RL) (Sec.~\ref{sec:MOD_FREE}).





% decluttering actions where non-target objects can be temporally stored in a separate holding space.

% They are symmetric along the z-axis,
% The shapes 
% and their shapes are known in advance.
% with respect to the gripper 

% At the core of our approach is the interplay between a model-based heuristic-guided RHP and a model-free NN with recurrent units trained with Reinforcement Learning (RL).
% The NN is trained to map observations into: 
% \i a distribution over the pose of the target object,
% \ii a stochastic policy
% \iii and its corresponding value function, 
% (Sec.~\ref{sec:MOD_FREE}). 

% In Fig.~\ref{fig:control}, we show an overview of our proposed approach.
% It consists of dynamically mapping data from the execution environment and task 
% priors into an abstract image-based representation of the observation, such that
% spatial information on occluded and observable spaces is maintained (Sec.\ref{sec:OBSER}). 
% Then, this observation is passed to the NN. 
% Conditioned by the observation history, the NN generates a 
% distribution over the probable poses of the target object.
% This distribution is combined with the current observation to 
% reconstruct likely initial states for RHP.

% The hybrid planner runs RHP, in a physics simulator, over each of these initial states
% where the policy and value heads of the NN are used as the RHP heuristic. The actions of highest value returned by the planner for each initial state are weighted by the likelihood of that state, and the action with highest expected return is executed (Sec.\ref{sec:HYB}). 
% This system is used again at every time step during execution, in a model-predictive control fashion.

% the NN iss used to generate a 
% The NN embeds the observation history into a latent belief vector $\hat{b}$ 
% and generates a distribution over the pose of the target object.
% The generative head of the NN 
% Conditioned by $\hat{b}$, the generative head of the NN is used to create 
% predicted distribution by the generative head of the NN over the 
% and the current observation are used to construct the most likely underlying states (Sec.\ref{sec:STATE_GEN}). 

% The framework is composed of two phases: first the heuristic learning phase which takes place in simulation, then the execution phase in which VisualRHP is interleaves the real-world actions with the physics simulator at run time. 
% We will begin by describing the execution phase (Sec.~\ref{sec:EXE}) assuming learning has already taken place, and then characterize the learning phase that makes it possible (Sec.~\ref{sec:HEU}). 


% \add{At execution time, a library of object types and shapes is assumed given. 
% Object recognition on the present scene detects poses and types. 
% In a real world, off-the-shelf tools could be used such as AR-markers, PoseCNN \cite{xiang2017posecnn}, DenseFusion \cite{wang2019densefusion}, etc.   
% In a simulated world this information readily available.
% This allows the system to place the correct shape, however complex, in the image-based representation of the observation.}
% We adopt quasi-static physics model. 
% The world state is not dynamic, in the sense that objects are always at rest unless they
% are in the robot’s gripper and the robot is moving.

%% -- Scratch -- %%
% A heuristic-guided RHP is then engaged over each of these predicted states, where 
% the policy and the value function are used as the RHP heuristic (Sec.\ref{sec:RHP}).
% The returned action that is expected to lead to the highest 
% future sum of discounted rewards, called \emph{return},
% is then resolved into the robot joint motion and executed in the real world (Sec.\ref{sec:ACT_SEL}).

% where the policy orients the searches towards higher
% higher return and the value head is used a proxy to estimate the return beyond the RHP horizon. 
% Depending on the complexity of the task, action selection can then be performed in one of two ways. 
% An action is either generated by a model-free stochastic policy (Sec.\ref{sec:MOD_FREE})
% or following a hybrid approach that performs heuristic-guided RHP on the most likely estimate of the environment state (Sec.\ref{sec:HYB}).
% The selected action is then resolved into the robot joint motion and executed in the real world.


% balances computation time with robustness to the evolution of complex system dynamics, 

% includes different clutter densities, object geometries, and desired object types.

% in the form of a stochartic policy or  
% Action generation is then condition by the learned belief spte.
% The first key idea is to map real-world sensory information and combine it with task to a colour-labelled image representation of the current observation.   
% I also This image allows to combine 

% is an mdp in which all
% rewards are negative, there is a set G ⊂ S of goal states, and the objective is to minimize the total
% expected cost (negative reward) incurred before reaching a state in G and terminating. We define
% cost function C(s, a) in the sspp to be −R(s, a) in the original mdp, so that all costs are strictly
% positive.

% \begin{figure*}[!t]
% \centering
% \includegraphics[max width=0.9\textwidth]{figures/control.pdf}
% \caption{Overview}
% \label{fig:control}
% \end{figure*}
% \captionsetup{labelformat=parens, justification=centering}
% \includegraphics[scale=0.13]{execution.png}
% \includegraphics[max width=\columnwidth, angle =-90]{figures/control.pdf}
% \includegraphics[max width=\columnwidth]{figures/control.pdf}
% \vspace{-4mm}

% $$
% \begin{aligned}
% r(s,a) = 
% \begin{cases}
% r_{invalid} \in \mathbb{R}_{\lll0},  & \text{if} \, \ T(s,a) \in S_{\textrm{invalid}} \\
% r_{valid} \;\;\: \in \mathbb{R}_{<0},   & \text{otherwise}.    
% \end{cases}
% \end{aligned}
% $$
%% \\ Scratch \\ %%

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/5-Hybrid.tex <==
\section{Decision Making Under Occlusion} \label{sec:OPC}
\subsection{Observation Space} \label{sec:OBSER}
It is essential to have an expressive representation of the observation
yet compact enough to keep the NN size relatively small as it will 
be queried multiple times per action selection.
Even though in the real world the camera is gripper-mounted, 
before we feed the observation into the NN,
we render it in a top-down view, 
% of the scene (
as shown in the top-left of Fig.\ref{fig:control},
% we render observations 
% in a top-down view of the scene 
making
the spatial relationships between objects and the geometry of 
occluded and observable areas more explicit.

We built on the abstract image-based representation 
of a fully observable environment in \cite{bejjani2019learning, bejjani2021learning}.
In addition to colour labelling objects based on their functionality (target in green, clutter in red, and surface edges in black),
we represent occluded and observable spaces by white and grey coloured areas respectively. 
% from is generated by a simple ray-tracing algorithm.
The geometry of the occluded areas is computed by illuminating 
the scene from the robot's camera perspective.
We use a black line to represent the shelf edge and brown 
for the shelf walls. 
The top-down view enables data from the execution environment and task priors to be combined.
% Object detection on the execution environment 
%     identifies the poses and types of visible objects in the camera FOV.
%     The objects' poses and types allow the simulation environment to place the correct object shape and colour in the abstract image-based representation of the observation.
%     The pose of the robot's gripper is computed from the robot forward kinematics.
% The task priors consist of observation-invariant information, 
%     including 
%     the type of the target object, the shape corresponding to every object type,
%     the shape of the shelf (walls and edge), 
%     the geometry of the gripper, 
%     and the camera FOV.
%     By including task priors in the representation, 
%     the learner does not need to remember them from the observation stream.
\begin{itemize}
    \item Object detection in the execution environment 
    identifies the poses and types of visible objects in the camera FOV.
    The objects' poses and types allow the simulation environment to place the correct object shape and colour in the abstract image-based representation of the observation.
    The pose of the robot's gripper is computed from the robot forward kinematics.
    \item The task priors consist of observation-invariant information:
    the type of the target object, the shape corresponding to every object type,
    the shape of the shelf (walls and edge), 
    the geometry of the gripper, 
    and the camera FOV.
    By including task priors in the representation, 
    the learner does not need to remember them from the observation stream.
\end{itemize}

% \footnote{ 
% When the execution environment is a realistically simulated world,
% objects' poses and types are readily available.
% If the execution environment is the real world, off-the-shelf tools could 
% be used (\eg, AR-markers, PoseCNN \cite{xiang2017posecnn}, DenseFusion \cite{wang2019densefusion}, etc.).}.  
% defined at the beginning of the task 
% and maintained until completion.  



\subsection{Hybrid Planner} \label{sec:HYB}
\begin{figure}[t]
%   \centering
  \includegraphics[width=0.5\textwidth]{figures/hybrid.pdf}
  \caption{Hybrid planner running two RHP queries,
  one for each peak represented by the contour lines (left).
  RHP is shown executing $2$ roll-outs of depth $3$ for each root state.}
  \label{fig:HYB}
%   \vspace{-0.5cm}
\end{figure}
% The hybrid planner queries the NN to generate  
% states with likely poses of the target object to be at the roots of RHP searches. 
% Then, the hybrid planner calls RHP over each of the root states to compute an action 
% to be executed at each root and its estimated \emph{return}.
% The action corresponding to the highest weighted return is executed.
The hybrid planner algorithm, presented in Alg.\ref{alg:HYB} and 
illustrated in Fig.~\ref{fig:HYB}, is detailed as follows:\\
\textbf{State Generation} (Alg.~\ref{alg:HYB}, line~\ref{l:genState}):
With information from previous observations
captured in the NN recurrent units,
% Primed by prior observations, 
the NN uses the current observation 
to generate an updated distribution over
target object pose. 
For each peak in the distribution,
the hybrid planner creates a root state with the target object placed at the peak location,
while the obstacle poses remain the same as in the current observation. 
The weight of a root state is
computed as the relative likelihood 
of its corresponding peak. 
It measures how likely it is for the target object to be found 
at the predicted location compared to the other potential sites.
RHP is then called over each of the root states (Alg.~\ref{alg:HYB}, line~\ref{l:queryRHP})
\\
\textbf{Occlusion-aware RHP} (Alg.\ref{alg:RHP}):
RHP performs $m$ stochastic roll-outs from root state $s_0$
up to a fixed horizon depth $h$ in the physics simulator. 
Each roll-out is executed by following the stochastic policy $\pi(\Bar{o})$ acting on the observation
history.
The \emph{return} $R_{0:h}$ of a roll-out is computed as the sum of the discounted rewards 
generated by the model and the expected return beyond the horizon estimated by the value function $V(\Bar{o}_h)$:
$
R_{0:h} =  r_1 +  \gamma r_2 + \ldots + \gamma^{h-1}r_{h} + \gamma^{h}V(\Bar{o}_h).
$
RHP returns the \emph{first} action $a_0$ and $R_{0:h}$ of the roll-out 
that obtained the highest \emph{return}. \\
% $R_{0:h}$ out of the $m$ roll-outs, 
% as well as the corresponding $R_{0:h}$ of that roll-out.
%Hence, 
%the RHP heuristic plays two roles:
%it informs the search through sampling, and as an %approximation of
%the rewards beyond the horizon.\\
\textbf{Action Selection} (Alg.~\ref{alg:HYB}, line~\ref{l:actSel}):
%%%%%% Wisdom comments %%%%%%%%%%%%%%%%%%%%%%
% The action to be executed by the robot is decided upon after performing the RHP queries.
% The return of an RHP query is scaled by the weight of its root state.
% The action to be executed is the one that is expected to lead 
% to the highest return while also balancing this expectation
% with how likely it is for the target object to be at the predicted location.
% To decide the robot's action, 
The \emph{return} of every RHP query is scaled by the weight of its root state (Alg.~\ref{alg:HYB}, line~\ref{l:scale}). Therefore, the robot picks the action that maximizes the \emph{return} with respect to both the probability of the roll-out, and the probability of the location of the target object.
% \setlength{\textfloatsep}{0.1cm}
% \setlength{\floatsep}{-1cm}
% \setlength{\textfloatsep}{-10pt}
% \setlength{\dblfloatsep}{-10ex}
% \begin{minpage}{0.48\textwidth}
% \begin{minipage}{\displaywidth}
% \begin{figure}[
% \begin{minipage}{0.3\textwidth}
\begin{algorithm}[t]
  \scriptsize
  \LinesNumbered
  \SetKwInput{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{trained neural network NN,
        observation history $\Bar{o}$, \qquad\qquad\qquad\qquad
        number of roll-outs  $m$, horizon depth $h$}
  \Output{action $a_r$}
    \textit{rootActions} $\leftarrow$ [ ], \, \textit{weightedReturns} $\leftarrow$ [ ] \\
    \textit{rootStates}, \textit{rootWeights} $\leftarrow$ generateStates(NN, $\Bar{o}$)\label{l:genState}\\
    \For{$s_o, w$ in [rootStates, rootWeights]}{
        $a_{r}, R_{0:h}$ $\leftarrow$ RHP(NN, $s_o$, $\Bar{o}$, $m$, $h$)\label{l:queryRHP}\\
        \textit{rootActions}.append($a_{r}$) \\
        \textit{weightedReturns}.append($w \times R_{0:h}$) \label{l:scale}\\
    }
    \textbf{return} rootActions[$argmax$(\textit{weightedReturns})] \label{l:actSel}
    \caption{Hybrid planner (NN, $\Bar{o}$, $m$, $h$)}
    \label{alg:HYB}
\end{algorithm}
% \end{minipage}]
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
  \scriptsize
  \SetKwInput{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{
         trained neural network NN,
         root state $s_0$, 
         observation history $\Bar{o}$, \qquad \qquad
         number of roll-outs  $m$, horizon depth $h$}
  \Output{action $a_0$, return $R$}
    $RolloutsReturn \leftarrow$ [ ], \,
    $FirstAction \leftarrow$ [ ] \\
    \For{$i$ = 1,2, \ldots, $m$}{
        $R \leftarrow 0$, \, $\Bar{o}_i \leftarrow \Bar{o}$ \\
        $s, \ o \leftarrow $ setSimulatorTo$(s_{0})$ \\
        $\Bar{o}_i$.append$(o)$\\
        \For{$j$ = 1,2, \ldots, h}{
            $a \sim \pi(.|\Bar{o}_i)$  \\      	
            \If{$j$ \textbf{is} 1}{
                $FirstAction$.append($a$)
            }
            $s, \ o, \ r \leftarrow$ simulatePhysics($s,a$) \\
            % $r \leftarrow$ receiveRewards \\ %receiveRewards($s_t$) \\ 
            $R \leftarrow R + \gamma^{j-1}r$ \\
            $\Bar{o}_i$.append$(o)$\\
            \lIf{isTerminal($s$)}{ 
                \textbf{break}
            }
          }
        \lIf{\textbf{not} isTerminal($s$)}{ 
            $R \leftarrow R + \gamma^{h}V(\Bar{o}_i)$
        }
        $RolloutsReturn$.append($R$)
    }
    % \textbf{return} $FirstAction[$argmax$(RolloutsReturn)]$, \\
    %                 \qquad \quad \  max$(RolloutsReturn)$
    \textbf{return} $FirstAction[$argmax$(RolloutsReturn)]$,  max$(RolloutsReturn)$
    \caption{RHP (NN, $s_o$, $\Bar{o}$, $m$, $h$) with an occlusion-aware heuristic}
    \label{alg:RHP}
\end{algorithm}   




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
% \begin{wrapfigure}{L}{0.49\textwidth}
% \begin{minipage}{0.48\textwidth}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}

% \hfill
% \end{minipage}
% \vspace{-12pt}
% \end{figure}



% \begin{algorithm}[t]
%   \LinesNumbered
% %   \SetAlgoNlRelativeSize{-3}
%   \SetKwInput{Input}{Input}
%   \SetKwInOut{Output}{Output}
%   \Input{Three-headed neural network NN, \qquad
%          observation history $\Bar{o}$,\qquad\qquad\qquad\qquad\qquad
%          no. of rollouts  $m$, horizon depth $h$}
%   \Output{action $a$}
%   \vspace{2mm}
%     \textit{rootStatesAct} $\leftarrow$ [ ]; \textit{rootStatesWeightedR} $\leftarrow$ [ ] \\
%     \textit{rootStates}, \textit{rootStatesWeights} = generateStates(NN, $\Bar{o}$)\label{l:genState}\\
%     \For{$s_o$, w in [rootStates, rootStatesWeights]}{
%         $a_o, R_{0:h}$ = queryRHP(NN, $s_o$, $\Bar{o}$, $m$, $h$)\label{l:queryRHP}\\
%         \textit{rootStatesAct}.append($a_0$) \\
%         \textit{rootStatesWeightedR}.append($w \times R_{0:h}$) \\
%     }
%     \textbf{return} rootStatesAct[$argmax$(\textit{rootStatesWeightedR})] \label{l:actSel}
%     \caption{Hybrid planner (NN, $\Bar{o}$, $m$, $h$)}
%     \label{alg:HYB}
% \end{algorithm}


% \begin{algorithm}[]
%   \LinesNumbered
%   \SetKwInput{Input}{Input}
%   \SetKwInOut{Output}{Output}
%   \Input{NN, 
%          root state $s_0$,
%          observation history $\Bar{o}$, 
%          no. of rollouts  $m$, horizon depth $h$}
%   \Output{action $a_0$, return $R_{0:h}$}
%   \vspace{2mm}
%     $RolloutsReturn \leftarrow$ [ ]; $FirstAction \leftarrow$ [ ] \\
%     \For{$m_i$ = 1,2, \ldots, $m$}{
%         $R \leftarrow 0$, \, $\Bar{o}_i \leftarrow \Bar{o}$ \\
%         $s, \ o = $ setSimulatorTo$(s_{0})$ \\
%         \For{h$_j$ = 1,2, \ldots, h}{
%             $\Bar{o}_i$.append$(o)$\\
%             $a \sim \pi(.|\Bar{o}_i)$  \\      	
%             \If{h$_j$ \textbf{is} 1}{
%                 $FirstAction$.append($a$)
%             }
%             $s, \ o \leftarrow$ simulatePhysics($s,a$) \\
%             $r \leftarrow$ receiveRewards \\ %receiveRewards($s_t$) \\ 
%             $R \leftarrow R + \gamma^{h_j-1}r$ \\
%             \If{isTerminal($s$)}{ 
%                 \textbf{break}
%             }
%           }
%         \If{\textbf{not} isTerminal($s$)}{ 
%             $R \leftarrow R + \gamma^{h}v(\Bar{o}_i)$
%         }
%         $RolloutsReturn$.append($R$)
%     }
%     \textbf{return} $FirstAction[$argmax$(RolloutsReturn)]$, \\
%                     \qquad \quad \  max$(RolloutsReturn)$
%     \caption{queryRHP (NN, $s_o$, $\Bar{o}$, $m$, $h$)}
%     \label{alg:RHP}
% \end{algorithm}



%% -- Scratch -- %%
% Weighing the return by the probability of its root state balances promising returns with how likely 
% it is for the desired object to be found at its predicted location. 
% computing the actions and the weighed estimate of the returns at the root states.
% The returns are weighed by the probability of their root states as measured from the KDE. 
% The action corresponding to the highest weighted return is executed by the robot. 

% The generative model, conditioned by the observations history produces a heatmap f 

% When reaching for the desired object

% replicating in the simulator potential states to be at the roots of multiple RHP queries. 

% A QMDP-net consists of two modules (Fig. 2). One encodes a Bayesian filter, which performs
% state estimation by integrating the past history of agent actions and observations into a belief. The
% other encodes QMDP, a simple, but fast approximate POMDP planner [18]. QMDP chooses the
% agent’s actions by solving the corresponding fully observable Markov decision process (MDP) and
% performing one-step look-ahead search on the MDP values weighted by the belief.


% The hybrid approach consist of querying a RHP over potential states with different desired object pose.
% Each RHP query return 

% heuristic-guided RHP that is rooted at the best estimate of the current state.
% In addition to the end-to-end learned policy and value function (similar to the previous section), the NN used in the 
% hybrid approach is also trained to estimate the actual state 
% of the environment from the observation history.

% Every tree nodes represents an observation and not a belief in our case.
% Actions are then selected by weighting the ?? with the belief \cite{karkus2017qmdp}
%% \\ Scratch \\ %%

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/6-Model-free.tex <==
\section{Training the Three-Headed NN} \label{sec:MOD_FREE}
% \begin{figure}[]
% \captionsetup[subfloat]{farskip=-5ex,captionskip=-5ex}
% \captionsetup[subfigure]{labelformat=empty}
%   \centering
%   \subfloat[]{\includegraphics[width=0.46\textwidth]{figures/NN.pdf}}
%   \caption{NN architecture.}
%   \label{fig:NN}
% \end{figure}
\begin{figure}[]
  \includegraphics[width=0.48\textwidth]{figures/NN.pdf}
  \caption{NN architecture.}
  \label{fig:NN}
\end{figure}

Prior to using the NN in the closed-loop decision making scheme,
the NN is trained in a physics simulation environment
(the same environment that will be used by the hybrid planner).
The NN must
(\emph{i}) generalize over variable number of objects and shapes in the observations,
\ii and maintain a belief from the observation stream
in order to 
predict the distribution over the target object pose 
and to generate an informed search and retrieve policy and value function
for RHP to use them as a heuristic.
The NN architecture that satisfies these conditions is illustrated in Fig.\ref{fig:NN}.
The first two components are a Convolutional Neural Network (CNN)
connected to LSTM units.
The CNN takes advantage of having an abstract image-based representation of the observation
to ensure generalization over object shapes and numbers.
The output of the LSTM layer, $\hat{b}$, summarizes the stream of CNN embeddings
into a latent belief vector. 
$\hat{b}$ is then passed through a feed-forward Deep Neural Network (DNN) 
that models the policy, another DNN for the value function, and 
a generative head 
for estimating the pose distribution
of the target object.
% for the target object pose distribution.
The generative head outputs a heat-map, $\hat{y}$, of size equal to the input image, 
where higher pixel values indicate higher chances that the target object is at that location.
As it is common to have the policy and value function sharing
some of NN parameters to stabilize the learning
% in applications where the visual input is significant 
\cite{mnih2016asynchronous, schulman2017proximal}, 
we also found that having the generative head sharing the CNN and LSTM components 
of the NN with the policy and value function acts as a regularizing element. 
% leading to greater stability in the learning process. 

Training a randomly seeded $\theta$-parametrized
NN with recurrent units over images
in a partially observable environment with complex physics 
and in a continuous actions space 
is particularly challenging \cite{mohammed2020review}. 
To increase the likelihood of convergence,
the learning algorithm
uses
% follows a sequential training process of IL, 
% followed by 
RL with a curriculum \cite{narvekar2020curriculum}.
% , where 
% task instances are gradually increased in complexity.
% \textbf{Imitation Learning:}
% In the first learning phase, we collect $P$ demonstrations, 
% in the form of state-action sequences 
% $\langle s_{0}, a_{0}, \ldots, s_{L-1}, a_{L-1}, s_{L} \rangle_p$ 
% where $L$ is the sequence length and $s_L$ is a terminal state.
% The demonstrations are genrated
% by solving random task instances using a Kinodynamic RRT planner over a fully observable version of the problem, that is, with $o \equiv s$.
% The NN is trained over the fully observable and sub-optimal demonstrations. 
% This learning phase is not enough to solve the problem under partial observability.
% Nevertheless, it offers RL a better starting point than a randomly seeded NN.
% \textbf{Curriculum-based Reinforcement Learning:}
% Next, we train the NN under partial observability with curriculum-based RL. 
The curriculum is constructed over three task parameterizations to gradually increase the clutter density and, by consequence, 
the occlusion in the environment.
The first parameterization
consists of environments with
random number of objects between $1$ and $4$.
The initial poses of the
target and clutter objects are sampled from a uniform distribution over the shelf. 
The next task parameterization uses between $5$ and $10$ objects.
% limits the minimum number of objects to $5$. 
The final task parameterization limits the minimum number of objects to $7$ 
and the pose of the
target object is sampled from a uniform distribution covering only the back half of the shelf.
Throughout the training, we use random polygon-shaped objects 
% (target and obstacles) 
for the NN to learn generalizable features. 

The policy and the value function are trained 
with synchronous Advantage Actor-Critic (A2C) \cite{wu2017scalable}.
% using the Proximal Policy Optimization
% (PPO) for the policy loss
% \cite{schulman2017proximal}. 
The generative head is trained in a supervised fashion.
The target $y$ for updating the generative head is  
a heat-map
showing the ground 
truth pose of the target object as given by the simulator. 
The combined loss function is, therefore:
\begin{align*}
& \mathcal{L}_{\textrm{}}(\theta) =
  \frac{1}{M} \sum_{i=1}^{M} 
    % -  Adv(\Bar{o}_i,\Bar{o}'_i)   \frac{\pi_{\theta}(a_i|\Bar{o}_i)} {\pi_{\theta_{old}}(a_i|\Bar{o})} \nonumber \\
    -  Adv(\Bar{o}_i,r_i,\Bar{o}'_i)  \;  \textrm{log}\pi_{\theta}(a_i|\Bar{o}_i)  \nonumber \\
    % -  \textrm{PPO}(Adv(\Bar{o}_i,\Bar{o}'_i), \   \frac{\pi_{\theta}(a_i|\Bar{o}_i)} {\pi_{\theta_{old}}(a_i|\Bar{o})}, \ \varepsilon) \nonumber \\
    & +  c_1 \;  (r_{i}+\gamma V_{\theta_{old}}(\Bar{o}'_i)-V_{\theta}(\Bar{o}_i))^2 \nonumber \\
    & -  c_2 \;  H(\pi_{\theta}(.|\Bar{o}_i)) \nonumber \\
    % +  c_3 \; \frac{1}{2}\sum_k(\hat{y}_k-y_k)^2,
    & -  c_3 \; \frac{1}{jk}\sum_{j,k}( y^{jk}_i\textrm{log}\hat{y}_\theta^{jk}(\Bar{o}_i) +  (1-y^{jk}_i)\textrm{log}(1-\hat{y}_\theta^{jk}(\Bar{o}_i)),
\label{eq:update_both}
\end{align*}
where $c_1$, $c_2$, and $c_3$ are hyper-parameters, $M$ is the batch size,
$H$ is the entropy term added to encourage exploration,
$j$ and $k$ are the heat-map pixel indices,
and 
$Adv$ is the advantage function estimate formulated over the observation history:
\begin{equation*}
Adv(\Bar{o}_i, r_i, \Bar{o}'_i) = r_{i} +\gamma V_{\theta_{old}}(\Bar{o}'_i)-V_{\theta_{old}}(\Bar{o}_i).
\end{equation*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \ie the environment is fully observable 
% shadows and the camera field of view are not rendered . 
% The NN is trained with IL to replicate the behaviour observed in the demonstrations, to estimate the value of a state if the RRT planner where to be engaged at that state, and to generate a distribution over the pose of the desired object\footnote{At this point in the training process the distribution is unimodal as the target object is always observable in the demonstrations.}.  \commentl{Again, I think we should cite our previus paper here, since this is common between the two.}

%\subsection{Curriculum-based Reinforcement Learning}

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/7-Experiments.tex <==
\section{Experiments} \label{sec:EXP}
We ran a number of experiments in a physics simulator
and in the real world.
% (video available on \textcolor{myblue}{https://youtu.be/khweZ4FXWfo}). 
The goals of the experiments are two-fold: 
(\emph{i}) to evaluate the performance of the proposed approach in dealing with occlusion and physics uncertainties,
\ii to verify the approach's transferability to retrieve different target objects in the real world.
% environments with different physics parameters. 

\subsection{Evaluation Metrics}\label{sec:EV_MET}
We select evaluation metrics that allow us to 
quantitatively measure the aforementioned goals.
(\emph{i}) The first metric is \emph{success rate}. 
% It is measured as the percentage of successfully completed tasks.
A task is considered successful if the target object is retrieved 
in under $50$ actions, the total task planning and execution time 
is under $2$ minutes, and none of the objects
are dropped off the shelf.
\ii As we also target real-time applications, 
the second metric is the 
\emph{average planning and execution time per task}.
\iii The \emph{average number of actions per task} is the third 
metric as the learning objective 
is to solve the problem with the minimum number of actions.




\subsection{The hybrid Planner and Baseline Methods}\label{sec:}
\textbf{Hybrid planner}: The NN is trained as in Sec.~\ref{sec:MOD_FREE}.
It takes a $64$$\times$$64$$\times$$3$ input 
image\footnote{We used robot-centric images, 
i. e., the colour-labelled abstract images track the
robot from the top-view perspective. 
We found that the robot-centric view reduces
the amount data required by the learning algorithm due to the symmetry of the scene when compared to a world-centric view.}. 
The CNN is composed of three consecutive layers of 
convolution, batch normalization, and maxpooling. 
We use $8$, $8$, $16$ filters of size $3$$\times$$3$ and strides $2$$\times$$2$. 
The CNN is followed by a single LSTM layer of $128$ units.
The policy head is composed of two dense layers with $128$ neurons each. 
The policy output layer has $8$ neurons corresponding to the means 
and standard deviations of the horizontal, lateral, rotational, and gripper actions. 
We use $tanh$ activation function for the means and $sigmoid$ for the standard deviation.
The value head has two dense layers with $128$ and $64$ neurons respectively, 
and a single neuron for the output with linear activation function.
The generative head follows a sequence of three upsampling and convolution layers. 
The filter sizes are 8, 8, 16 and $3$$\times$$3$. 
The final layer is a $64$$\times$$64$$\times$$1$ convolution layer with 
linear activation function followed by a 
$sigmoid$ function to decode the heat-map.
% The heat-map is decoded by passing the final layer through a sigmoid function.
Except for the output layers, we use a $leaky\ relu$ activation throughout the network.  
The NN is updated using the RMSProp optimizer in TensorFlow \cite{tensorflow2015-whitepaper}. 
We use the PPO formulation for the policy loss function \cite{schulman2017proximal}. 
Following the proposed training curriculum, the difficultly of the task is increased every time the success rate of the hybrid planner with $m$=$4$ and $h$=$4$ exceeds $80\%$. 
The training is terminated once the success rate converges. 
We use the following learning parameters: 
% $P$=$10,000$, 
$learning\ rate$=$0.00005$, $c_1$=$0.5$,
$c_2$=$0.01$, $c_3$=$1.0$, $\gamma$=$0.995$, 
and $M$=$1500$.
% , and $\varepsilon=0.075$.
% During IL,
% the $Adv$ is set to 
% $V_{\theta_{old}}(\Bar{o}) + lowest MC return   Because the rewards are strictly negative$.
% the positive value of $0.5$.
% The set the KDE bandwidth to $0.25$.
We compare three versions of the hybrid planner with $m$ and $h$ RHP parameters of $2$$\times$$2$, $4$$\times$$4$, and $6$$\times$$6$.
\\
\textbf{Hybrid planner limited}: Instead of performing weighted evaluations of multiple RHP queries, 
this baseline only evaluates the most likely target pose and executes the predicted action.
We implement it with $m$=$4$ and $h$=$4$.
\\
\textbf{Greedy}: This policy presents a deterministic model-free approach. 
The NN is trained similarly to our approach 
excluding the generative head from the architecture.
The robot is directly controlled by the policy head of the NN (without RHP). 
Actions are defined by the mean of the action distribution outputted by the 
policy head over the continuous planar actions space.
It is inspired by 
\cite{novkovic2020object}.
% \cite{hausknecht2015deep, igl2018deep, novkovic2020object}.
% \rm{We also evaluate an additional greedy policy, Greedy$_{gen}$, that uses the NN trained with the generative head.
% The purpose is to investigate if 
% the NN will learn a better representation for the policy head, when also trained to generate the target object pose distribution.}
\\
\textbf{Stochastic}: 
This policy is a stochastic version of the greedy policy. 
Actions are sampled from the policy output.
As shown in \cite{jaakkola1995reinforcement},
RL trained stochastic policies provide higher \emph{return} than deterministic ones in a POMDP.
\\
\textbf{Stochastic$_{\mathrm{gen}}$}: We also evaluate an 
additional stochastic policy that samples the policy head
of the NN trained with the generative head.
The purpose is to investigate if 
the policy learns a better reasoning
about the target object pose distribution
when trained using our proposed approach.
\\
% the NN will learn a better 
% policy if trained
% representation for the policy head when 
% also trained to generate the target object pose distribution.
% learn good reasoning about the target object pose distribution. 
% \\
% Since the hybrid planner relies on stochasticity in the roll-outs,
% this baseline allows us to isolate the 
% effect of stochasticity on the behaviour independently from the look-ahead planning.
%First, it is oriented toward finding deterministic policies, whereas the optimal policy is often stochastic, selecting different actions with specific probabilities (e.g., see Singh, Jaakkola, and Jordan, 1994).
\textbf{Hierarchical planner}: This approach offers a model-base baseline.
The low level plans are generated either with kinodynamic RRT \cite{haustein2015kinodynamic} or following a hand-crafted heuristic.
The low level plans are executed in open-loop.
The high level planner has access to the following actions: 
Search( ): positioned outside the shelf,
the robot moves from the far left to the far right of the shelf while pointing the camera inwards.
Throughout this motion, information is collected
on the pose and type of detected objects.
Rearrange($Obj_i$): move a certain object to a free-space in the back of the shelf
by planning 
with Kinodynamic RRT on collected information from the previous Search action.
Move$\_$out( ): rotates the robot to face the inside of the shelf, 
then moves the robot out following a straight line heuristic. 
Retrieve($Obj_i$): plan with Kinodynamic RRT on available information to reach, grasp, and pull-out the target object. 
The high level planner is outlined in Alg.~\ref{alg:HIE}.
This baseline is an adaptation of \cite{dogar2014object}.
\begin{figure}
\captionsetup[subfloat]{farskip=-2pt,captionskip=-4pt}
\captionsetup[subfigure]{labelformat=empty}
\hspace*{-1.1em}
\subfloat[]{ \includegraphics[width=0.162\textwidth]{tikz/sr_objNb_occlu.pdf} }\hspace*{-0.45em}
\subfloat[]{ \includegraphics[width=0.162\textwidth]{tikz/t_objNb_occlu.pdf}  }\hspace*{-0.45em}
\subfloat[]{ \includegraphics[width=0.162\textwidth]{tikz/ac_objNb_occlu.pdf} }

\hspace*{-1.1em}
\subfloat[]{ \includegraphics[width=0.162\textwidth]{tikz/sr_noisy_occlu.pdf}  }\hspace*{-0.45em}
\subfloat[]{ \includegraphics[width=0.162\textwidth]{tikz/t_noisy_occlu.pdf}   }\hspace*{-0.45em}
\subfloat[]{ \includegraphics[width=0.162\textwidth]{tikz/ac_noisy_occlu.pdf}  } 

\hspace*{-0.7em}
\subfloat[]{ \includegraphics[width=0.495\textwidth]{tikz/legend_occlU.pdf}  }

\caption{Performance \wrt different clutter densities and noise levels.}
\label{exp:sim}
\end{figure}

\begin{algorithm}[t]
% \small
\scriptsize
\While{target object \textbf{not} retrieved}{
    Search( )\\
    \eIf{target object \textbf{not} located}{
        Rearrange(\textit{closest object to robot})\\
        % \quad \quad 
        % \textit{free-space in the shelf's back})\\
        Move$\_$out( )\\
        }
    % \lElse{
    {
        Retrieve(target object)
        }
}
\caption{Hierarchical planner}
\label{alg:HIE}
\end{algorithm}


\subsection{Simulation Experiments}
\begin{figure}[b]
  \centering
  \includegraphics[width=0.49\textwidth]{figures/noiseFig_v2.pdf}
  \caption{Snippets of the current observation with noise level=0.15. Task solved with Hybrid$^{4\times4}$.}
  \label{fig:noiseSeq}
\end{figure}

\begin{figure*}[!t]
\captionsetup[subfigure]{labelformat=empty}
\subfloat[]{ \includegraphics[width=1.0\textwidth]{figures/real_seq_vinegar.pdf} }\vspace{-10pt}
\\
% \vspace{-10pt}
\subfloat[]{ \includegraphics[width=1.0\textwidth]{figures/real_seq_horseradish.pdf} }\vspace{-10pt}
\\
% \vspace{-0pt}
\subfloat[]{ \includegraphics[width=1.0\textwidth]{figures/real_seq_marierose.pdf}  }
% \hspace*{-1.25em}
\caption{Snapshots of the hybrid planner retrieving different target objects.}
\label{fig:seq2}
\vspace{-16pt}
\end{figure*}

\textbf{Setup: }
We use two Box2D physics simulators \cite{box2D}, 
one acting as the execution environment 
and the other as the simulation environment where RHP is performed.
% As the execution environment, we use the two-dimensional Box2D \cite{box2D} physics engine, which is also the physics engine used by RHP.
The experiments are conducted on
% We use 
an Intel Xeon E5-26650 computer equipped with an NVIDIA Quadro P6000 GPU.
The experiments evaluate the performance \wrt 
increased clutter density and increased noise level on 
the shape and physics parameters in the execution environment.
The increase in clutter density is aimed at challenging 
the robot with higher occlusion ratios
and more complex multi-object interactions.
% The clutter density ranges from $0$ to $10$ obstacles. 
% The shapes of the objects are randomly generated within the constraint 
% of being small enough to be at least directionally graspable.
The increase in the noise level addresses modelling  errors
% errors on the physics and shape parameters
between the execution environment and the simulation environment.
% transferability of an approach
% to environments with different physical parameters.
% from the environment is was trained in or planned over to another environment. 
Noise is added on the parameters of an object before the execution of an action.
The noise is generated from a Gaussian distribution centred  
around the mean of the object's density $1$ $kg/m^2$ and friction 
coefficient $0.3$. 
% \rm{and vertices around the object's centre within $0.1\ cm$ and $5.0\ cm$ in range.}
Additionally, the shapes of the objects are altered by adding noise on the coordinates of an object's vertices \wrt its centre of mass.
We evaluate the performance over noise levels with standard deviation ranging from $0.0$ to $0.25$ with random number of obstacles up to $10$. 
An experiment with noise level = $0.15$ using Hybrid$_{4\times4}$ is shown in Fig.\ref{fig:noiseSeq}.
% The initial poses of the objects are sampled from a uniform distribution over the shelf.
The width and depth of the shelf are W:$50$$\times$D:$35\ cm$. 
The dimensions of the gripper are modelled after a \emph{Robotiq 2F-85} gripper
% \footnote{https://robotiq.com/products/2f85-140-adaptive-robot-gripper} 
mounted on a \emph{UR5} robot.
% \footnote{https://www.universal-robots.com/products/ur5-robot/}. 
\\

\textbf{Results: }
The results are shown in Fig.\ref{exp:sim}.
Each data point in the results is averaged over $300$ task instances with random object configuration.
In terms of success rate, we observe a decreasing trend \wrt clutter density and higher noise levels. 
This is expected as the task becomes more challenging
with higher occlusion ratio and changing dynamics. 
The hybrid planner 
% \rm{, with all its parameterizations,} 
outperforms the other baselines. 
Its success rate improves with higher number of roll-outs and horizon depth as evident by the higher success rate of Hybrid$^{6\times6}$ compared to Hybrid$^{2\times2}$.
% Under the RHP parameters ($4$$\times$$4$), 
Performing a weighted evaluation over the predicted 
poses achieves a slightly higher success rate than just evaluating the most likely one.
% as thorougher and deeper search is performed.
Furthermore, the stochastic policies outperform the greedy policy. 
This improvement may be the result of the additional information gained from a stochastic motion.
The stochastic and greedy policies exhibit similar success rates with higher noise levels. 
This is because the changes in physics and object shapes introduce enough randomness in the system
for the greedy policy to act in a similar fashion to the stochastic policy.
% Nevertheless, the stochasticity alone is not enough to justify the higher success 
% rate of the hybrid planner.
% \rm{The greedy$_{gen}$ did not result in a significant difference to its greedy counterpart. 
% Hence, training the additional 
% generative head of the NN did not result in an improved representation for the policy.}
The stochastic$_{\mathrm{gen}}$ results are slightly better than its stochastic counterpart, but the difference is not big enough to draw any major conclusion.
The hierarchical planner suffers from the sharpest drop in success rate in both experiments. 
The open-loop execution often fails to produce the intended results.

The average time per task shows a clear advantage for the model-free approaches (greedy, stochastic, and stochastic$_{\mathrm{gen}}$).
Actions are generated almost instantaneously. 
% and execution time is only limited by the physics simulation.
The hybrid planner time degrades with more exhaustive RHP searches.
% Since the RHP heuristic can generate actions in real-time, the hybrid planner 
% allocates most of its computation time simulating the physics of the roll-outs.
The difference between Hybrid$^{4\times4}$ and Hybrid$^{4\times4}_{\textrm{lim}}$ 
is not significant despite the latter achieving lower time per task.
This result indicates that the hybrid planner does not often generate a large number 
of potential positions for the target object which would have otherwise resulted
in a bigger time difference.
The hierarchical planner average time is on par with the Hybrid$^{6\times6}$ planner.
These results indicate that simulating the physics during planning 
is the computation bottleneck in a contact-rich environment.


Except for the hierarchical planner, all of the 
approaches perform a similar number of actions per task.
Evidently, the stochastic policies
perform slightly worse than the hybrid planner, 
while the greedy policy is the most efficient.
% the stochastic policy performs slightly worse than the hybrid planner.
The hybrid planner, despite relying on stochastic roll-outs, 
executes fewer actions than the stochastic policies as decision 
making is better informed with RHP.
The scale of the number of actions for the hierarchical planer is highly dependent
on the parameters of the underlying low level planners. 
Nevertheless, with a high noise level and clutter density, the high level planner increasingly calls 
the low level planner for re-planning.
% in order to correct for the un
% which results in a higher action count.







% \captionsetup{font=normalsize}
% \caption{Performance \wrt clutter density.}
% \label{exp:t_clutterDensity}
% \captionof{figure}{Performance \wrt clutter density.}
% \end{minipage}

%% -- Scratch -- %%
% \ii to assess its ability to generalize to random environment settings,
% We compare our approach to state-of-the-art inspired baselines that we designed 
% to run in a partially observable environments with continuous control:
% \begin{itemize}
%     \item  \emph{Stochastic policy}: This baseline looks
% \end{itemize}

% \textbf{Methods:}\\
% \textbf{Task:}\\
% Easy\\
% Moderate\\
% Hard\\
%% \\ Scratch \\ %%






==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/8-Real-3DSim.tex <==
\section{Realistic Experiments} \label{sec:3D}
The simulation results show that the hybrid planner can be reliably used in environments with 
different physics parameters.
To further validate this finding, we test our approach in a realistic setup.
We use the 3D MuJoCo physics engine with the Deepmind Control Suite \cite{tassa2020dmcontrol}
as the execution environment, and Box2D as the simulation environment for the hybrid planner.
% The camera in mounted om the gripped with $25^0$ tilt angle.

To replicate a conservative performance of real-world object detection tools 
from a single image in clutter \cite{wang2019densefusion, xiang2017posecnn},
% (\eg, AR-markers, PoseCNN \cite{xiang2017posecnn}, DenseFusion \cite{wang2019densefusion}, etc.),
the execution environment (having access to the ground truth) would only report 
to the simulation environment 
the poses and types of objects whose more than $50\%$ of their body 
is visible within the current camera view.
% Object detection is outside the scope of this work.
% It is a well studied field and $50\%$ could be considered a conservative estimate.
% Object detection in a single image
% is already a very well studied problem
% Otherwise, an object is considered 
% we consider an object detectable in the execution environment if more than $50\%$ of its body is visible,
% \ie, the simulation environment only received the poses and types of currently detectable objects in the execution environment.

We use $m$=$4$ and $h$=$4$ as they offer a reasonable balance 
between success rate and execution time.
The shelf dimensions are W:$50$$\times$D:$35$$\times$H:$30 \ cm$.
We conduct 30
tasks with random number of obstacles, up to 10.
% 20 randomly sampled low (4 objects) and highly (9 objects) cluttered scenes. 
We also experiment with the stochastic policy 
as it showed the second best success rate in the previous experiments.
% For each task, we use the hybrid policy and the stochastic policy. 
% Experimental results are in Table~\ref{table:real_world_results_table}. 

The hybrid planner and the stochastic policy achieve a success rate of $88\%$ and $79\%$, respectively.
These results are similar to the previous experiment with high noise levels.
% We performed experiments under different clutter densities.
% Snapshots of the resulting behaviour are shown in Fig.\ref{fig:seq1} and Fig.\ref{}.
Examples of tasks solved with the hybrid planner are shown in Fig.~\ref{fig:seq1}, Fig.~\ref{fig:snapshots}, and in the attached video. 
% A video showing the performance  is available in the supplementary material.
The hybrid planner demonstrates that 
% it can control the robot for searching 
% and retrieving the target object. 
when the target object is not visible, 
the robot 
performs information-gathering actions by advancing into the shelf 
and manipulating obstacles to increase visibility.
% intentionally advances into the shelf while pushing
% the clutter around. 
% exhibiting an interactive search behaviour.
When the robot loses sight of a previously detected target object,
due for example to an obstacle blocking the camera view,
the robot focuses its search 
on the area where the target object was last seen.  
% The robot is shown to recover from situations where an obstacle
% falls within the gripper fingers.
% Furthermore, once the target object is grasped, 
% the robot manoeuvres its way backwards while avoiding 
% pushing obstacles off the shelf. 
% The robot's behaviour shows that the
% NN 
% heuristic that is driving the planner 
% stores relevant knowledge on past
% observed objects. 
% which are not anymore detected.

% In this work, ``realistic'' refers to a 3D physics simulator, Mujoco \cite{mujoco} used 
% with the Deepmind Control Suite \cite{tassa2020dmcontrol}.
% 3D physics simulator which is designed to
% mimic the real-world.
% The location of robot base is empirically optimised to minimize the robot body colliding with the shelf. 

% \begin{figure}[h]
%   \begin{center}
%   \includegraphics[width=1.0\textwidth]{figures/seq10.pdf}
%   \end{center}

% \end{figure}

%   \centering
%   \begin{subfigure}{.3\linewidth}
    % \includegraphics[width=1.0\textwidth]{figures/seq12.pdf}
%   \end{subfigure}
    % \hfill
%   \begin{subfigure}
    % \includegraphics[width=1.0\textwidth]{figures/seq10.pdf}
%   \end{subfigure}
%   \caption{Snapshots of the hybrid planner retrieving the green object.}



==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/8.8-Real-World.tex <==
\subsection{Real-World Experiments} \label{sec:3D}
To validate the simulation results,
we conducted a number of real-world experiments using 
the hybrid planner
for retrieving
a variety of everyday objects (oil bottle, tomato box, jars, oat box, vinegar bottle) from a cluttered shelf.
% From the previous section, we know that our 
We used $m$=$4$ and $h$=$4$ as the 
previous section have showed that 
these parameters offer a reasonable balance 
between success rate and execution time.
We mounted an RGB camera
on the end-effector of a \emph{UR5} 
with a \emph{Robotiq 2F-85} gripper 
and manually calibrated the hand-camera transformation. 
We used the Alvar AR tag tracking library for object poses and types detection \cite{Alvar}.
We used Box2D as the simulation
environment to run the hybrid planner.
The shelf dimensions are W:$50\times$D:$35\times$H:$40 \ cm$.
Snapshots from these experiments are shown in 
Fig.~\ref{fig:seq1} and Fig.~\ref{fig:seq2}.
A video of these experiments 
% attached.
is available on
\textcolor{myblue}{https://youtu.be/dY7YQ3LUVQg}.

We conducted a total of 30 experiments
with up to 8 objects. The robot achieves
a success rate of 90$\%$ with an average of 50 seconds per experiment.
The robot exhibits an informed search behaviour 
by executing actions that increase the
visibility of previously unobserved spaces and by manipulating objects to 
reveal occluded areas behind them. 
In the experiment where the robot is tasked with retrieving the oil bottle,
the robot first approaches the middle of the shelf and searches 
the area behind the oat box. Once the oil bottle is spotted, 
the robot goes around the
cereal box, losing sight of the oil bottle, 
then reaches again for the oil bottle from a less 
cluttered direction.
In the second experiment where the robot is tasked with retrieving the 
vinegar bottle,
we observe the importance of a reactive behaviour when the bottle slips from the
robot's grasp.
The robot is able to recover from this situation by reopening the gripper, approaching
the bottle, and then re-grasping it and pulling it out of the shelf.
In the experiment where the robot is tasked with retrieving the
horseradish jar, the robot pushes obstructing objects to clear an
approach for grasping and retrieving the jar.

Two failed cases were due to the inverse kinematics solver
failing to map an action from the end-effector planar Cartesian space to the robot joint space.
A potential future solution would be to mount 
the robot arm
on a mobile base and leverage the additional gain in
Degrees of Freedom.
Another failure was attributed
to the hybrid planner failing to 
grasp a jar target object
wedged in the corner between the shelf wall 
and 
another obstacle object.


% is available on
% \textcolor{myblue}{https://youtu.be/4iSsogfCkMc}.
% The robot behaviour in the real world is reminiscent to what we
% observed in the realistic experiment. 



==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/9-Conclusion.tex <==
\section{Conclusions} \label{sec:CONC}
% We described a hybrid planning approach for retrieving a target object 
% from a cluttered shelf under occlusion.
% We described a hybrid approach that combines the sequential reasoning over the physics
% offered by model-based methods
% with the scalability of 
% model-free methods in partially observable environments.
The experiments have shown the efficiency and transferability
of our approach in challenging environments.
The robot's behaviour validates that the
NN stores relevant information from past
observation to guide future actions.
%----------
% In comparison to the other baseline approaches, the hybrid planner can
% react in near real-time while also accounting for complex physics 
% interactions under occlusion.
Despite being limited to 2D planar actions,
it offers a stepping stone towards
% real-world 
applications such as object retrieval from fridges 
and supermarket shelves with limited height.

This work forms a solid foundation for extending 
the hybrid planner to 3D manipulations actions 
where the robot can move along the z-axis.
We intend to use tags-free object pose detectors 
in clutter to allow for greater
flexibility~\cite{xiang2017posecnn, wang2019densefusion}.
Additionally,
we envision using an abstract colour-labelled 3D voxelized 
representation of the space with 3D-CNN and 
% recurrent neural 
transformer
architectures.
% \clearpage
% We showed that by trading a small computation time for informed decision making, 
% the robot can reliably retrieve a target object
% from challenging environments.
% In this work, we used fixed values for the number of roll-outs and the horizon depth.
% To save on computation time, we intend to extend this work to dynamically adjust these parameters 
% according to semantic and spatial features in the environment.

% A 2D planer solution to such tasks
% can be immediately useful.

% However, it is limite

% The hybrid approach model-free representation of the of the target object pose and a heuristics 
% for look-ahead planning 
% 1- 3D
% 2- dynamically adjusted RHP parameters

% We presented a hybrid planner that uses
% an occlusion-aware heuristic for retrieving a target object in a physics environments.

% The experiments validated the effectiveness of combining model-based and model-free approaches
% to handle occlusion uncertainty and multi-object physics interactions. 
% This work forms a solid foundation for extending the hybrid planner to 3D manipulations actions
% such that the robot can lift 
% We intend to further develop this work to use colour-labelled 3D voxelized representation of the space.


% \add{Other similar scenarios include fridges and supermarket shelves with limited height. 
% A 2D planer solution to such tasks
% can be immediately useful.}
% In this work, we propose a method 
% for searching and retrieving a target object,  in real-time, from a cluttered environment with occlusions.

    % \item \textit{Manipulation under partial observably requires reasoning over the temporal correlation between the observation history and future actions.}
    % Interactive search is defined as leveraging manipulation action for information gathering. 
    % In a cluttered environment, the robot can 
    % move obstacles blocking a sensor Field of View (FOV) or move the sensor itself to get a better view of the scene.
    % In a cluttered environment, the robot must account for object interactions that might take place outside the sensor FOV while the robot is moving. Also, maintaining information on previously searched spaces and detected objects are essential for efficiently finding and retrieving a desired object.  
    
    % We avoid hard coding what and how previously observed features in the scene should be remembered. 
    % Instead, We take a learning approach to interactive search. 
    % Using a meticulously devised learning curriculum, 
    % the robot learns how to map observation history to actions.

% \rm{
% showed that by trading a small computation time for informed decision making, 
% the robot can reliably retrieve a target object
% from environments with different physics parameters.
% Alternative approaches showed a robust behaviour in low clutter environment.
% However, because of occlusion, it is not always possible to know a priori the clutter density.
% The model-free approaches can be most useful in time-critical applications, 
% but less so if the cost of failure is too high.
% The model-based approach can be reliably used where it is more likely to find collision free-trajectory, \eg, decluttering objects from the front of the shelf.
% In this work, we used fixed values for the number of roll-outs and the horizon depth.
% To save on computation time, we intend to extend this work to dynamically adjust these parameters 
% according to semantic and spatial features in the environment. }



% We presented a model-free mapping from observation history to a distribution over likely states, 
% action distribution, and value estimate.
% We showed showed that this mapping enables physics-based reasoning under occlusion.
% We validated our claim in a experiments conducted in different physics environments.

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/corrections.tex <==
Assumption:
We assume that all of the objects are unions of convex polyhedra that are extrusions along the z axis (that is, they have a constant horizontal cross-section) and that their shapes are known in advance.

The world state is not dynamic, in the sense that objects are always at rest unless they are in the robot’s gripper and the robot is moving.

perception service attempts to detect instances of the known shape models

we assume that there is no identity uncertainty, that is, the perceived identities of objects are correct and unique.

Limitations:

---------------------------------------------------------------------------------
---------------------------------------------------------------------------------

+ explicitly differentiates between regions
- table-top: simplistic
+ baseline were thorough
+ simple and effective

error on creating the 2-D representation regarding object pose, shape, and type.
It is indicated that no prior knowledge is assumed about the objects
raw image from the in-hand camera is used to infer all of this information to create the 2-D representation

Does it ever output the wrong shape? 
small ... it matter even if it were wrong?
see scenes with very differently sized objects, and not just primitive shapes

extended to truly 3-D environments
go up or down relative to the table
The observability representations used are strictly 2-D
2 shelves, one target
genuine pile of objects
How will you scale your method to these (more realistic) scenarios? It’d be great to discuss in the paper.

video: at least one of the baselines is shown also

I think performance will definitely degrade as noisy real images are not going to produce as clean of representations as can be achieved in simulation. 

+ But the core ideas of the algorithm set the stage for applying it in these more complicated settings.

---------------------------------------------------------------------------------
---------------------------------------------------------------------------------

- it is essentially planar

- Observations for the system aren’t noisy, beyond the fact that if an object is not 50\% visible, it is not considered.

- Does the algorithm take care of toppling displaced objects?
  trained in a 2D How realistic is that? stacking, object shapes vary with height. 
  dynamics as flat or high objects will behave differently
  
- high clutter picking non-target objects might be totally unavoidable

- objects very simple. generalize to more real/complex shapes? Adding those in testing to see performance would help.

- introduction = related work section, without highlighting, explaining or motivating the proposed approach until the very end.

- Before related work, make more clear what is the problem and approach proposed. 
  For instance, it isn’t clear that this paper cares about not dropping objects from a shelf until section 3.

- During intro RHP are assumed known, add short explanation.

- In line 107, “We do not assume any prior knowledge on the number, pose, and shape of the objects on the shelf.”  
  Object shape in training affect the results. extremely simple, suffer: real with diverse shapes and textures.

- cannot perform well with scenes that have many more than 10 objects, as these scenarios do not appear in training and are also not tested.

- Line 109 “single optimization problem with the objective of minimizing the total number of actions.”,  
  doing nothing would be the best policy.
  
- How is the “type” of an object described? Specially if there is now prior knowledge on the shapes or objects, how can the algorithm reason over that?

- Line 125 is not obvious “we opt for a uniform negative reward per action, casting the problem as a stochastic shortest path”. What is “uniform negative reward”? Does uniform here refer to a uniform distribution or just a constant? What is the implication of it being a stochastic shortest path?
    Response: A stochastic shortest-path problem(sspp) hS, A, T, C, Gi is an mdp in which all
    rewards are negative  (See definition 2 in ``Integrated task and motion planning in belief space'')
            
- Fig. 3 is rather simple and not enough to understand the complete approach. For instance, the role of previous observations is missing, or how RHP is used.

- Line 150, how is it possible to represent objects in an image if no prior knowledge of the shape is known (as said in line 107)? An image obtained from the in-hand camera would not be able to provide shape information beyond the pixels it can capture. However, the example observation in Fig 3. does show knowledge of the full geometry of the objects. It is unclear how task prior can help on that without really knowing having access to prior knowledge on the objects. Even the accumulation of observations woulndt be enough to tell what is the shape of an object at the back of the shelf.
  Response: Agree, shapes should be moved to task priors.

- The generated raw images are noise free which makes them unrealistic to render in a real scenario. Especially if again there is no prior knowledge on object shapes, real depth images will be noisy and correcting for that without prior shape information seems difficult.

- The paper relies on access to a simulator from which it is possible to render the effect of the actions taken during RHP. However, in a real scenario, this simulator and rendered images are unlikely to be accurate, which could largely hurt the approach.

- How does the algorithm account from objects falling from the shelf? Is it just by having a sparse reward like the one that marks zero if an object fails or the target is not reached, and 1 otherwise?

- Line 234, what does “data point” refer to in this sentence?

- Line 253, the greedy baseline is unclear. Why is the mean of the action a good idea? Why is this helping to understand the value of predicting target pose distribution?

- I would make sense to have a baseline that takes the most likely target pose and performs the predicted action for that pose.
 Response: Will do so

- Line 282, could you clarify this: “vertices around the object’s centre within 0.1 cm and 5.0 cm in range.”?

- In line 289, what does it mean “with all its parametrizations”?

- In the realistic experiments, the set of observations is still rendered as in the training/2D planar case? What objects are used? Same as in the 2D case?

- Video: It would be nice to include something that represent which action was selected. maybe an arrow for motion and something different when gripper is closing.

- RW: There is much more complexity in the real world than just different physics parameters.


==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/icra_rev.tex <==
training the three-headed NN:
    1) this type of loss has existed out there, such as in the work [Kei Kase, etc. Transferable Task Execution from Pixels through Deep Planning Domain Learning, ICRA2020]; 
    2) Using RNN to perform implicit belief updating has also been widely used in RL community.

RHP: planning is actually an evaluation for the learned policy

The planning is then not motivated well, why not just run the learned policy? 

Without the supervised loss, the policy may not learn good reasoning about the target object pose distribution. 

RHP planning is a biased approximation to the learned policy

It is not clear about how the target object’s position is sampled in the testing, which actually also affects all methods’ performance, especially to the biased RHP planner.

more than 10 (maximum in training)

If the target object is changed, or the target objects are very different in shape

this work requests the objects with the same height and the robot movements in the 2D space
 
it is not clear how each object’s polygon-shape is
sampled during the training

---------------------------------------------------------------
---------------------------------------------------------------

but is not preferable when it comes to time spent

assumptions/inputs to the approach would be more clearly stated

How is the search query represented?

(given multiple objects of the same “type” exist in the shelf)	Would this just be outsourced as a new “type”?

This will require an externally calibrated camera sensor.

The abstract image-based representation is world-instead of ego-centric. Have you experimented with an ego-centric representation 

it would also help if NN/V/pi would be written as an input.

p. 2: “Since the state of is not always accessible”

----------------------------------------------------------------
----------------------------------------------------------------
what exactly is the observation space?  
Is the (simulated) camera RGB only, or does it contain depth?  
What exactly is the action space?  
How is the library of object type-shape pairs represented, 
and how does the system know which object is the target?
- A framework for push-grasping in clutter.  Mehmet R. Dogar and Siddhartha S. Srinivasa, RSS 2011.
- Robot Grasping in Clutter: Using a Hierarchy of Supervisors for Learning from Demonstrations.  Michael Laskey, Jonathan Lee, Caleb Chuck, David Gealy, Wesley Hsieh, Florian T. Pokorny, Anca D. Dragan, and Ken Goldberg, CASE 2016.

p2:  "approaches sated so far"
p2:  "the state of is not always"
p5, Alg 3.  "end" before "else"
p4. Alg 1.  Wouldn't it be simpler (and equivalent) to just
store the best action so far?
p4, Alg 2.  After $R \gets R ...$, what is $^1 r$?
Ref [14,34] errors
Video at 0:14  "eperiements"

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/iros_rev.tex <==
REV 18405 : ++
1) (reality gap): Added sentence to Introduction Section, RHP paragraph + added reference to PhD thesis for more details
2) (action space definition): Introduction Section, Assumptions paragraph (last)
3) (clarification on performance): DONE


REV 18413 : +
1. The occlusion in test scene is simple, the performance
of the algorithm in more clutter scenes needs to be
verified.
2. This paper is well-writing except the planner part,
which is hard to understand.
3. It is a pity that there is no follow-up discussion on
the failure cases caused by corners,I think that a new type
of interaction can be introduced to solve it. 

REV 20761: +
1)  2D planar actions is a strong limitation 
2) Why A2C not SAC
3) Compare with baseline [27]
4) RL learning details

REV 21157: --
1) LSTM: length of the sequence
2) Having a look at the video which includes both the real
scene and simulation environment, it is not clear how the
green object appears in the simulation even though it is
not yet seen in the real setting. Since it is mentioned
that the generative head for object pose is trained in a
supervised manner, how is it labelled while executing the
RHP in test time.
3) training details
4) how is the position of the object
extracted from the pixel intensities?

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/meta_reviews.tex <==
3. Please summarize your comments. (Visible to author after author notification)
This paper addresses the problem of finding a known target object in clutter through physical rearrangement of objects. The paper presents a hybrid model-based, model-free approach for performing this operation in an explicit POMDP model of the task.

All reviewers acknowledge the importance and difficulty of the target task.

Reviewer #2 finds the method to be essentially a combination of existing techniques designed for this task, while reviewer #3 finds the presentation too unclear to articulate exactly what the novelty of the method is over existing work.

The reviewers bring up significant concerns about the complexity of the environment, namely that all objects have the same height and similar shape, greatly simplifying the problem. This is further complicated by no simulated camera noise in the experiments making them far from reality. While the reviewers bring up the scenario of grocery shelves as a possible place where the shape and height assumptions are valid, this is a much more specific application than those claimed in the paper and still suffers from the need to deal with highly variable object appearance and materials such as metal cans or transparent containers that can be IR absorbent rendering depth cameras difficult to use without significant processing.

All reviewers also note that the paper's claims of requiring no prior knowledge of the objects is misleading, as at least knowledge of the class of object shape primitives is present in design of the algorithm / learning.

Furthermore, the highly idealized simulation examples are rendered much weaker in the context of related work on actual physical systems with variable object shapes such as the "Mechanical Search" work from Goldberg's lab which is not cited in the submitted paper (see http://ai.stanford.edu/mech-search/)

As such I recommend rejection of the paper.

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/notes.tex <==
%#############################
%#############################
TODO (after submission!)
expected sum of the \emph{return} --> expected \emph{return}  VVVVV
$\Bar{o}_i$.append$(o)$ update its location in algo    VVVV
the advantage should have r_i in it    VVVVVV
use $\mathcal{O}^i$ in hierarchical rearrange and retrieve  VVVV
The stochastic and greedy policIES exhibit similar   VVVVV
We use $m$=$4$ and $h$=$4$ as THEY OFFER a reasonable balance VVVVV
Examples of tasks solved with the hybrid planner are SHOWN in VVVV
and in the attached video --> in the experiments' video    -------
connecting state to observation is  the observation probability distribution $\Omega : S \times O \rightarrow [0,1]$  -------
long action sequences becomes impractical REMOVE S from become VVVVV
Since the state of is not always IN METHODOLOGY
They tackle top-down bin decluttering by removing obstructings
%#############################
%#############################

ICRA
why 2D is useful and important
shape variance (figures to show noise)

Add a brief description of RHP in the Introduction
Make the introduction sound less like Related Work
Clearly state the contribution of the work relative to previous work
Make the tracking the distribution over the target object pose more central

ADD: state dimention is variable, number of object is not known a priori.
RL IL
%#############################
%#############################
meta reviews:
- novelty is unclear, combination of existing work
- complexity of the environment, object shape, camera noise
- object appearance and materials such as metal cans or transparent containers are hard to detect
- no prior knowledge? at least knowledge of the class of object shape primitives is present!
- highly idealized simulation examples

%#############################
%#############################
Rev3: (I don't understand what he understood from our approach)

- If the state vector is of variable size, how does the RL algorithm deal with that? 
- The RHP seems to have access to a physics simulator. That makes the statement also weird. Being able to simulate the environment offline to do (heuristic)planning means there is full god-like knowledge of the whole scene.

- why not go completely model-free (ans: it is a baseline)

- object seems to be disappearing between frames (ans: if more than 50/100 is occluded, then they are not detectable and hence disappear) 

- task priors? (ans: the explanation is clear in the text and in the figure!)

- How good is the policy after Imitation learning? How good is the pose-estimator? (ans: add IL baseline? but this has been adressed in previous work)

- Sharing parameters is not about the "significance" it is about having "Compatible Features" representations between the policy and value function, return to Sutton for more details.
%#############################

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/plots_two_col.tex <==
\begin{figure*}[t]
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{sr_objNb}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=11, ymin=50, ymax=100,
    ylabel={Success rate \%}, xlabel={Number of obstacles}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0.0,-0.5)},anchor=south west,legend columns=7, draw=none, opacity=0.0, font=\scriptsize},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]     table[x index=0,y =hyb6,col sep=comma]   {sr_0.dat};
 	\addplot [blue,          line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]      table[x index=0,y =hyb4,col sep=comma]   {sr_0.dat};
 	\addplot [blue!50!white, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb2,col sep=comma]   {sr_0.dat};
 	\addplot [orange!90!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {sr_0.dat};
  	\addplot [red!70!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {sr_0.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {sr_0.dat};
 	\addplot [green!60!black, line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]   table[x index=0,y =sto,col sep=comma]    {sr_0.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {sr_0.dat}; 
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy60) at (axis cs:0,60) {};
	\node (sy70) at (axis cs:0,70) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy90) at (axis cs:0,90) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:10,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy70) -- (ex |- sy70);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy90) -- (ex |- sy90);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{t_objNb}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=11, ymin=0, ymax=100,
    ylabel={Time in seconds}, xlabel={Number of obstacles}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize, 
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb6,col sep=comma]   {t_0.dat};
 	\addplot [blue,           line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb4,col sep=comma]   {t_0.dat};
 	\addplot [blue!50!white,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb2,col sep=comma]   {t_0.dat};
 	\addplot [orange!90!black,line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {t_0.dat};
  	\addplot [red!70!black,   line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {t_0.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {t_0.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid, scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {t_0.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {t_0.dat}; 
% 	\addlegendimage{empty legend}
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy20) at (axis cs:0,20) {};
	\node (sy40) at (axis cs:0,40) {};
    \node (sy60) at (axis cs:0,60) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:10,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy40) -- (ex |- sy40);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{ac_objNb}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=11, ymin=0, ymax=35,
    ylabel={Number of actions}, xlabel={Number of obstacles}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize,
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb6,col sep=comma]   {ac_0.dat};
 	\addplot [blue,           line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb4,col sep=comma]   {ac_0.dat};
 	\addplot [blue!50!white,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb2,col sep=comma]   {ac_0.dat};
 	\addplot [orange!90!black,line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {ac_0.dat};
  	\addplot [red!70!black,   line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {ac_0.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {ac_0.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {ac_0.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {ac_0.dat}; 
 	\legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy5) at (axis cs:0,5) {};
	\node (sy10) at (axis cs:0,10) {};
    \node (sy15) at (axis cs:0,15) {};
    \node (sy20) at (axis cs:0,20) {};
    \node (sy25) at (axis cs:0,25) {};
    \node (sy30) at (axis cs:0,30) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:10,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy5) -- (ex |- sy5);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy10) -- (ex |- sy10);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy15) -- (ex |- sy15);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy25) -- (ex |- sy25);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy30) -- (ex |- sy30);
\end{tikzpicture}
% \vspace{-20pt}
\end{minipage}
% \caption{Performance \wrt clutter density.}
% \label{exp:clutterDense}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
% [-1ex] 
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{sr_noisy}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=0.25, ymin=50, ymax=100,
    ylabel={Success rate \%}, xlabel={noise levels}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]   table[x index=0,y =hyb6,col sep=comma] {sr_n.dat};
 	\addplot [blue, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]            table[x index=0,y =hyb4,col sep=comma] {sr_n.dat};
 	\addplot [blue!50!white,   line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]   table[x index=0,y =hyb2,col sep=comma] {sr_n.dat};
 	\addplot [orange!90!black, line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]  table[x index=0,y =hyb4_lim,col sep=comma] {sr_n.dat};
  	\addplot [red!70!black,    line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]  table[x index=0,y =gre, col sep=comma] {sr_n.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]  table[x index=0,y =gre_hm,col sep=comma] {sr_n.dat};
 	\addplot [green!60!black, line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]  table[x index=0,y =sto, col sep=comma] {sr_n.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}] table[x index=0,y =mod, col sep=comma] {sr_n.dat}; 
    % \legend{Greedy, Greedy$_{gen}$, Stochastic, Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hierarchical}
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy60) at (axis cs:0,60) {};
	\node (sy70) at (axis cs:0,70) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy90) at (axis cs:0,90) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:0.25,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy70) -- (ex |- sy70);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy90) -- (ex |- sy90);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}
% \vspace{-8pt}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{t_noisy}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=0.25, ymin=0, ymax=100,
    ylabel={Time in seconds}, xlabel={noise levels}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize, 
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb6,col sep=comma]   {t_n.dat};
 	\addplot [blue,          line width=0.8pt, mark=diamond*, mark options={solid},scale=0.8]    table[x index=0,y =hyb4,col sep=comma]   {t_n.dat};
 	\addplot [blue!50!white, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb2,col sep=comma]   {t_n.dat};
 	\addplot [orange!90!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {t_n.dat};
  	\addplot [red!70!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {t_n.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {t_n.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {t_n.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {t_n.dat}; 
    % \legend{Greedy, Greedy$_{gen}$, Stochastic, Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hierarchical}
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\addlegendimage{empty legend}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy20) at (axis cs:0,20) {};
	\node (sy40) at (axis cs:0,40) {};
    \node (sy60) at (axis cs:0,60) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:0.25,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy40) -- (ex |- sy40);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}%
% \vspace{-8pt}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{ac_noisy}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=0.25, ymin=0, ymax=35,
    ylabel={Number of actions}, xlabel={noise levels}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize,
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb6,col sep=comma]   {ac_n.dat};
 	\addplot [blue,          line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb4,col sep=comma]   {ac_n.dat};
 	\addplot [blue!50!white, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb2,col sep=comma]   {ac_n.dat};
 	\addplot [orange!90!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {ac_n.dat};
  	\addplot [red!70!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {ac_n.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {ac_n.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {ac_n.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {ac_n.dat}; 
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy5) at (axis cs:0,5) {};
	\node (sy10) at (axis cs:0,10) {};
    \node (sy15) at (axis cs:0,15) {};
    \node (sy20) at (axis cs:0,20) {};
    \node (sy25) at (axis cs:0,25) {};
    \node (sy30) at (axis cs:0,30) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:0.25,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy5) -- (ex |- sy5);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy10) -- (ex |- sy10);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy15) -- (ex |- sy15);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy25) -- (ex |- sy25);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy30) -- (ex |- sy30);
\end{tikzpicture}
\end{minipage}
\caption{Performance \wrt different clutter densities and noise levels.}
\label{exp:sim}
\end{figure*}

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/response.tex <==
We would like to thank the reviewers for their thorough analysis, and address the main questions raised. 

- R1 “It is indicated that no prior knowledge is assumed about the objects […] The 2-D representations shown in the figures [...] look very clean to me.” R2 “how is it possible to represent objects in an image if no prior knowledge of the shape is known (as said in line 107)?”  

We apologize for the confusion on object shapes. When we indicated that no prior knowledge is assumed about the objects, we should have clarified that it only refers to the neural network (NN), which is trained with randomized arbitrary shapes. However, during execution, the overall system is given a library of object types and shapes. Object recognition on the present scene detects poses and types. This allows the system to place the correct shape (however complex) in the intermediate abstract representation. This abstract representation is then fed into the NN. 

- R1 “Does it ever output the wrong shape?” “It will be more compelling to see scenes with very differently sized objects.” R2 “How can this approach generalize to more real/complex shapes?” 

Object shape at execution time doesn’t need to exactly match object shape during training. We should have clarified that we do inject noise in the objects’ shape in the experiments of Fig. 6. This is what we meant by “vertices around the object’s centre within 0.1 cm and 5.0 cm in range” (which R2 asked us to clarify). To add noise onto the shapes, each vertex of an object gets a new coordinate in the object frame at every action step. The new coordinate is sampled from a Gaussian distribution centered at the initial coordinate of that vertex. By changing the Gaussian standard deviation from 0.05 (low noise) to 0.25 (high noise), we observed variation in the vertex coordinate anywhere between 0.1 cm and 5.0 cm w.r.t. to its initial location (in this experiment circles are replaced with octagons). For example, under high noise, an octagon object will have a very arbitrary shape.  

- R1 “It would be helpful to include some discussion about how this could be extended to truly 3-D environments.” R2 “The approach is trained in a 2D scenario, and even in Mujoco, the scenes are practically planar. How realistic is that?” 

We acknowledge that currently the approach solves 2D problems. However, we note that (i) planning under partial observability is a significant challenge in such multi-object environments, even in 2D; (ii) there are some practical problems, particularly shelves with limited height e.g. in supermarket shelves, where the current 2D planner can be immediately useful; (iii) our work is novel in proposing to learn to predict the possible locations of the hidden object, to deal with the partial observability, which we think is a useful contribution to solving this important problem; (iv) this idea of learning to predict the belief state seems applicable to 3D as well, e.g. using colour-labelled voxelated representations for the space and objects, which we leave as future work.  We also note that there were some admittedly limited 3D features of our system. Our realistic experiments were conducted in a 3D simulator, where the length of the shadow behind each object is affected by the relative height of the in-hand camera to the top of the objects.   

R2:  

- “It would make sense to have a baseline that takes the most likely target pose and performs the predicted action for that pose”  

We indeed experimented with this method during the development of this work. We don’t think it is a “baseline”, in the sense that it is still using the NN predictions about the hidden object location, and therefore is a variation of our method. The experiments showed that this variation achieved a slightly lower success rate, and therefore, in the paper, we used the proposed weighting scheme. We also note that, on average, our system generates 1.3 potential positions for the target object, and therefore the resulting planning and execution time are quite similar in practice. 

- “the distribution of training shapes for instance will clearly affect the results at test time. [...] Same with number of objects, there is no reason to believe that this approach can perform well with scenes that have many more than 10 objects”  

We agree that the distribution used in training must be somewhat representative of the shapes the system will see during execution. This is unavoidable in machine learning. However, the approach, in principle, is not limited to certain shapes or a predefined number of objects, thanks to the generalization provided by the training of the CNN. 

- “What is “uniform negative reward”?”, “How does the algorithm account from objects falling from the shelf?”  

We apologize this was unclear. By “uniform”, in this context we indeed mean constant. That is, we do not design more articulated reward functions that encode hints of what we think is the solution (as in reward shaping). Consequently, each no-terminal action has the same negative cost, and the problem is therefore a shortest-path problem. When an object, during training, falls off the shelf, the episode ends with an additional large negative reward.  

- “However, in a real scenario, this simulator and rendered images are unlikely to be accurate, which could largely hurt the approach.”  

This is a crucial aspect of our approach. The use of the learned policy and value function allows the planner to work on a short horizon, which allows fast MPC-like replanning at every time step.  Thus, we minimize compounding errors due to such inaccuracies (e.g. simulator or object detection inaccuracies). The abstract representation is updated at every iteration. 

- “Line 234, what does “data point” refer to” 

 It refers to the data points of the experiments’ plots in Fig. 6. 

- “If there is enough clutter and environment constraints, picking non-target objects might be totally unavoidable in order to retrieve a target goal.”  

The system can indeed learn to perform actions that are like two-fingered gripping, to move objects out of the way, as shown in Task 4 in the video. 

- “In the realistic experiments, the set of observations is still rendered as in the training/2D planar case? What objects are used? Same as in the 2D case?”  

In the realistic experiments, we used 3D boxes and cylinders. They had different dimensions from the objects used during training. 

- “Line 253, the greedy baseline is unclear. Why is the mean of the action a good idea?” 

The policy is represented as a Gaussian by the NN. Picking the mean of this Gaussian gives us the most likely action that maximizes the expected return, according to the network.  

- “Why is this helping to understand the value of predicting target pose distribution?” 

We wanted to see if training the network to predict the target pose distribution would create a latent representation that also helps with learning a better policy. 

==> Occlusion-Aware Search for Object Retrieval in Clutter IROS2021 - Compiled/reviews.tex <==
3. Please summarize the paper, state what you think the contribution is, comment on its strengths and weaknesses, and give advice for improving the paper.
The paper provides a hybrid model-free/model-based approach to doing object retrieval in partially observed cluttered table-top environments, both 2-D and 3-D. The model-based component is a receding horizon planner (i.e. model predictive control scheme) that takes an initial environment state and uses a physics simulator to execute actions generated by a stochastic policy previously learned in a model-free RL fashion in simulation. The model-free component predicts the initial state that the model-based component is initialized with. The state representation is specific to this table-top manipulation setting and is a 2-D abstract image showing the shapes and poses of objects (both a target object to be grasped and the other objects causing clutter), the boundaries of the environment, and importantly for this partially observed setting, different colorings for regions that are known to be free space and regions that have not been observed yet. This is an extension of previous work that assumed fully observable scenes. This abstraction is learned with a neural network from raw RGB image observations, where an LSTM recurrent neural network is used for the policy/value function learning to accommodate a history of observations and cope with the partial observability. There is also an image generator output head that produces a kernel density estimate of where the target object to be grasped is located in the scene. This heuristically guides the action selection. The policy learning is based on a curriculum such that it starts learning with a small number of objects and works its way up to ~10 objects in the scene causing significant clutter.

The paper is very clearly written. I like the abstract representation that is generated from observations, particularly that it explicitly differentiates between regions it has observed to be free space and regions that it has not yet observed due to occlusions. While the representation is perhaps optimized for this specific setting of table-top manipulation and the environments are simplistic, I think demonstrating its efficacy even in this simple environment is a good contribution, and the baseline algorithms in the experiments were thorough enough to show the proposed hybrid planner is successful. This to me seems like a relatively simple and effective way to handle partial observability for these environments. I advocate for acceptance and give some minor feedback as follows to improve the paper.

I would be interested to see more information about the error on creating the 2-D representation (especially from the 3-D environment) regarding object pose, shape, and type. It is indicated that no prior knowledge is assumed about the objects and the raw image from the in-hand camera is used to infer all of this information to create the 2-D representation. The 2-D representations shown in the figures and video look very clean to me. I could see though how there could be ambiguity working just from RGB images, especially if low-resolution images are input to the network, e.g. a cylinder from a low-profile straight-on view can look like a box. Does it ever output the wrong shape? And since the objects appear to all have similar dimensions, would it matter even if it were wrong? I think it will be more compelling to see scenes with very differently sized objects, and not just primitive shapes but more complicated object meshes that you would find in the real world.

It would be helpful to include some discussion about how this could be extended to truly 3-D environments. I realize a 3-D simulator is used in the experiments, but the objects are all located on a planar surface and the objects are all the same height. Also the robots actions are effectively in the plane, it does not go up or down relative to the table. The observability representations used are strictly 2-D. How will you extend to 3-D if you now have say a bookshelf with 2 shelves, and there is clutter on both levels but still just one target object to find. Or if the clutter is not so singulated and you have a genuine pile of objects to sift through. This presumably also complicates the action space more as there will be many more possibilities to be explored. How will you scale your method to these (more realistic) scenarios? It’d be great to discuss in the paper.

Small corrections:
Pg. 1, Paragraph 1: “Autonomously manipulating everyday objects…”
Pg. 5, 7.1, “... and none of the objects are dropped…”
Is the batch size correct? It’s reported in experiments Section 7.2 that batch size is 15,000. That seems quite large for image-based data

------------------------------------------------------------
POST REBUTTAL
Thank you to the authors for addressing our concerns. In view of the rebuttal comments and discussions with reviewers, I think the method is a nice extension of citation [14] to operate in partially observable tabletop environments where a top-down view is not possible and object models are not known. The biggest improvement to the paper would be to have experiments with real object meshes (e.g. objects from YCB dataset). In this case the primitive shape approximations will impose more error in the representation relative to the real world. Also doing this with a more realistic camera model and lighting conditions (preferably doing the experiments on a real platform) would be more compelling.

It should also be clarified in the paper about what prior information is used in training and execution. Specifically, discuss further the library of primitives being used. It is misleading to say "no prior information" was used as having candidate primitive shapes in training or to choose from at execution is a shape prior. Probably better to say known object models are not required, and are approximated with shape primitives. The real mesh experiments would then validate whether this approximation is okay in this setting.
4. Was the video submission useful? What was good about it? What could be done to improve it? (Write N/A if there was no video submission)
The video was good in that it showed the core task being performed, and I especially liked that it showed what the planner was reasoning over at every timestep, and how the observation representation was evolving. It's nice that multiple executions are shown, but they are not qualitatively very different so I felt it was a bit redundant watching the entire video. It would be more helpful to show one execution where at least one of the baselines is shown also, especially if there are interesting qualitative differences in the baselines that fail compared to the hybrid planner.
5. If code was submitted, we ask that you perform a sanity check. We do not ask that you run the code. But if you do, please comment on this too. Authors have been instructed to provide a readme file that points to the part of the code that needs to be peer-reviewed. Please, read this part of the code and answer the following questions: a) Does the code appear to implement the algorithm described in the paper? b) Did the readme file allow you to identify relevant parts of the code? c) Were you provided with data to replicate the results? Please, remember that code is for peer-review only and that you are not allowed to use this code outside the review process. (Write N/A if there was no code submission)
N/A
9. Comment on the potential impact of the paper to real robotics problems (taking COVID-19 impact into account). Please check the supplement material for the COVID-19 response.
I do not doubt that this method would work in the real world, though I think performance will definitely degrade as noisy real images are not going to produce as clean of representations as can be achieved in simulation. Surely manipulation in clutter and partial observability is crucial for real world manipulation. I think the task as performed in the experiments is perhaps a little contrived, one would expect more object size variability and a less uniform distribution of objects in e.g. a kitchen cupboard. But the core ideas of the algorithm set the stage for applying it in these more complicated settings.
12. Overall recommendation:
Weak Accept
13. Rate your level of confidence in this recommendation:
High
Reviewer #2
Questions
3. Please summarize the paper, state what you think the contribution is, comment on its strengths and weaknesses, and give advice for improving the paper.
A . Paper summary and contributions

This paper aims at solving the problem of picking a target object from a shelf, in a mostly planar setting, without dropping objects from the shelf.

It contributes by:
(i) Proposing a hybrid planner that first predicts a pose distribution of the target objects as well as, policy values and actions.
(ii) The most likely poses are then evaluated using RHP. The resulting best policy value when weighted by the likelihood of each pose is executed in an MPC fashion.

The approach is only tested in simulation, it is essentially planar, and the shape of the objects is reduced to circles, squares and triangles. Observations for the system aren’t noisy, beyond the fact that if an object is not 50% visible, it is not considered.

B . Positive aspects of the paper

The paper acknowledges the importance of dealing with cluttered environments where noise and uncertainty can arise in several dimensions including motion of objects or observations with limited information on the state.
The paper evaluates the approach on a different simulator and is capable of producing a performance of 88% in a novel simulator.

C. Feedback on the paper

Does the algorithm take care of toppling displaced objects?

The approach is trained in a 2D scenario, and even in Mujoco, the scenes are practically planar. How realistic is that? In many cluttered environments, stacking is quite common. Or simply, object shapes vary with height which is not contemplated in this work. Moreover, the simplification of 2D can cause further problems when learning the dynamics as flat or high objects will behave differently under pushing actions for instance.


If there is enough clutter and environment constraints, picking non-target objects might be totally unavoidable in order to retrieve a target goal. However this paper seems unable to deal with such scenarios.

The objects considered are far from realistic and very simple. I only observed cylinder-like rectangles, circles and triangles. How can this approach generalize to more real/complex shapes? Adding those in testing to see performance would help.

On the introduction, right now it reads more like a related work section, without highlighting, explaining or motivating the proposed approach until the very end.

Before going into the related work, it would suggest to make more clear what is the problem and approach proposed. Otherwise it is hard to follow the reasoning behind the structure and content of the related work. For instance, it isn’t clear that this paper cares about not dropping objects from a shelf until section 3.

During intro and related work, RHP are assumed known, however I would expect that many readers would benefit from a short explanation.


In line 107, “We do not assume any prior knowledge on the number, pose, and shape of the objects on the shelf.” However the distribution of training shapes for instance will clearly affect the results at test time. Specially when the objects considered are extremely simple, this is likely to suffer when objects are more real with diverse shapes and textures. Same with number of objects, there is no reason to believe that this approach can perform well with scenes that have many more than 10 objects, as these scenarios do not appear in training and are also not tested.

Line 109 says that “single optimization problem with the objective of minimizing the total number of actions.”, however this should mention that the actual goal is to retrieve a target, not just perform a minimum number of actions, where doing nothing would be the best policy.

How is the “type” of an object described? Specially if there is now prior knowledge on the shapes or objects, how can the algorithm reason over that?

Line 125 is not obvious “we opt for a uniform negative reward per action, casting the problem as a stochastic shortest path”. What is “uniform negative reward”? Does uniform here refer to a uniform distribution or just a constant? What is the implication of it being a stochastic shortest path?

Fig. 3 is rather simple and not enough to understand the complete approach. For instance, the role of previous observations is missing, or how RHP is used.

Line 150, how is it possible to represent objects in an image if no prior knowledge of the shape is known (as said in line 107)? An image obtained from the in-hand camera would not be able to provide shape information beyond the pixels it can capture. However, the example observation in Fig 3. does show knowledge of the full geometry of the objects. It is unclear how task prior can help on that without really knowing having access to prior knowledge on the objects. Even the accumulation of observations woulndt be enough to tell what is the shape of an object at the back of the shelf.

The generated raw images are noise free which makes them unrealistic to render in a real scenario. Especially if again there is no prior knowledge on object shapes, real depth images will be noisy and correcting for that without prior shape information seems difficult.

The paper relies on access to a simulator from which it is possible to render the effect of the actions taken during RHP. However, in a real scenario, this simulator and rendered images are unlikely to be accurate, which could largely hurt the approach.

How does the algorithm account from objects falling from the shelf? Is it just by having a sparse reward like the one that marks zero if an object fails or the target is not reached, and 1 otherwise?

Line 234, what does “data point” refer to in this sentence?

Line 253, the greedy baseline is unclear. Why is the mean of the action a good idea? Why is this helping to understand the value of predicting target pose distribution?

I would make sense to have a baseline that takes the most likely target pose and performs the predicted action for that pose.

Line 282, could you clarify this: “vertices around the object’s centre within 0.1 cm and 5.0 cm in range.”?

In line 289, what does it mean “with all its parametrizations”?

In the realistic experiments, the set of observations is still rendered as in the training/2D planar case? What objects are used? Same as in the 2D case?

The paper would benefit from discussing what are the main failure cases of their approach. What happens in that 10% of cases that can’t be solved.
4. Was the video submission useful? What was good about it? What could be done to improve it? (Write N/A if there was no video submission)
The video is useful, and quite easy to follow even before reading the paper. It would be nice to include something that represent which action was selected. maybe an arrow for motion and something different when gripper is closing.
5. If code was submitted, we ask that you perform a sanity check. We do not ask that you run the code. But if you do, please comment on this too. Authors have been instructed to provide a readme file that points to the part of the code that needs to be peer-reviewed. Please, read this part of the code and answer the following questions: a) Does the code appear to implement the algorithm described in the paper? b) Did the readme file allow you to identify relevant parts of the code? c) Were you provided with data to replicate the results? Please, remember that code is for peer-review only and that you are not allowed to use this code outside the review process. (Write N/A if there was no code submission)
N/A
9. Comment on the potential impact of the paper to real robotics problems (taking COVID-19 impact into account). Please check the supplement material for the COVID-19 response.
I believe this paper is not ready to be implemented in a real robotic platform and achieve the same level of performance.
While the authors say: "To our approach, the real world would be just another execution environment which we do not know its exact physics parameters.” There is much more complexity in the real world than just different physics parameters.
Real image observations are much more noise, and object shapes are more complex than the tested ones. Moreover, assuming planar scenarios is not realistic as objects have different height and vertical shapes which changes their dynamics.
12. Overall recommendation:
Weak Reject
13. Rate your level of confidence in this recommendation:
High
Reviewer #3
Questions
3. Please summarize the paper, state what you think the contribution is, comment on its strengths and weaknesses, and give advice for improving the paper.
The paper proposes a hybrid-scheme of model-free RL and heuristic-based planning for learning to act in a partially observable and visually cluttered environment in order to find and retrieve certain target objects. This combination is done in the spirit of Play Online Learn Offline (POLO) [14], albeit by replacing the trajectory optimization part with a heuristic-based search. The paper presents benchmarks on a simulated setup and compares it to a few baseline variants.

# Strengths:
----------------
* The paper attempts to solve a hard problem in general and does so while relying on visual input. The results while limited do show a working algorithm. The paper brings together different concepts from state-of-the-art to solve a significant challenge in robotics.

# Weakness:
-----------------
* The paper seems to gloss over many important details in my opinion. The presentation is often not clear. Some parts are very text-verbose and still somewhat confusing. As a suggestion, consider drawing a simple schematic to simplify the description of how all these moving parts come together. Another way is to introduce a bit more structure and divide the presentation of the algorithm to multiple smaller problems.

# Major Comments:
--------------------------
The following points follow no clear order of importance.

* The paper mentions that no priors about the number of objects or their shapes and poses. This claim raises two points:
1)- Is the state vector of variable size, since it contains some parameters from every object in the scene and some might be occluded in the beginning. If the state vector is of variable size, how does the RL algorithm deal with that? That seems like a non-standard RL setting. If not then this statement is somewhat misleading.

2)- The RHP seems to have access to a physics simulator. That makes the statement also weird. Being able to simulate the environment offline to do (heuristic)planning means there is full god-like knowledge of the whole scene.

* What is meant by task priors? I don't think this term has been clearly defined anywhere in the paper.

* I think it is crucial to be able to see the learning performance of the pose-estimator in order to provide a sanity-check for this part of the approach. Also, some testing of how this estimator may generalize would be great. In the video, the target object seems to be disappearing between frames while planning, I am not sure what that is a sign of.

* Sharing parameters is not about the "significance" it is about having "Compatible Features" representations between the policy and value function, return to Sutton for more details.

* Another significant point is the role of Imitation Learning. How good is the policy after Imitation learning? How good is the pose-estimator? It is important to show this baseline, in order to make the point that the RL/planning is actually improving something. Also, 10000 Samples of imitation pairs sound like a lot when considering that this has to be executed on a real robot. It would be interesting to see how the performance scales with the number of demonstrations and with their absence.

* It seems that approach needs the ground truth to train the pose-estimator. This is a major drawkback in my opinion. Having access to such information kind of undermines the whole endeavor. It is also not clear to me at all why the process of learning the pose-estimator is coupled with RL.

* RHP appears to be using the predictors learned via RL, value function, and pose-estimator. The paper mentions that these generally only return informative actions for a couple of time steps in a model-free setting. Why are they then used offline to do planning over a long horizon? I understand that planning in the space images is hard, but I don't see the motivation for not going completely model-free. Or at least I do not see why the planning performs well, while using quantaties approximated while doing RL. It is important for the authors to clarify this point.

* Has the experiment where the model-free approach is tested alone been tuned for best performance, or did the authors just adopt the best hyperparameters that worked for their approach and use them in the model-free scenario?

* Please add evaluations of sample complexity and learning behavior when comparing to model-free RL. It is not clear to me how many real samples one experiment/task has taken. I think this is a crucial indicator of applicability in a real scenario.

* A general question: Is there any sense in which this approach is actually solving a POMDP in the classical sense, i.e. is taking information-gathering actions? It would be interesting to highlight such behavior.


# Minor Comments:
---------------------------
* The paper refers to the proposed method as a "robust manipulation", that seems like a vague term. Can you expand on this?

* line 14: everyday-day

4. Was the video submission useful? What was good about it? What could be done to improve it? (Write N/A if there was no video submission)
The video is of very good quality.
5. If code was submitted, we ask that you perform a sanity check. We do not ask that you run the code. But if you do, please comment on this too. Authors have been instructed to provide a readme file that points to the part of the code that needs to be peer-reviewed. Please, read this part of the code and answer the following questions: a) Does the code appear to implement the algorithm described in the paper? b) Did the readme file allow you to identify relevant parts of the code? c) Were you provided with data to replicate the results? Please, remember that code is for peer-review only and that you are not allowed to use this code outside the review process. (Write N/A if there was no code submission)
N/A
9. Comment on the potential impact of the paper to real robotics problems (taking COVID-19 impact into account). Please check the supplement material for the COVID-19 response.
I think the problem the paper is tackling is important but I feel that the paper is missing too many details and leaves many open questions in general.

Also, the applicability in a real setting is not clear given some missing information about sample complexity and the need for a ready simulation of the environment.
12. Overall recommendation:
Weak Reject
13. Rate your level of confidence in this recommendation:
High

==> corrections.tex <==
Assumption:
We assume that all of the objects are unions of convex polyhedra that are extrusions along the z axis (that is, they have a constant horizontal cross-section) and that their shapes are known in advance.

The world state is not dynamic, in the sense that objects are always at rest unless they are in the robot’s gripper and the robot is moving.

perception service attempts to detect instances of the known shape models

we assume that there is no identity uncertainty, that is, the perceived identities of objects are correct and unique.

Limitations:

---------------------------------------------------------------------------------
---------------------------------------------------------------------------------

+ explicitly differentiates between regions
- table-top: simplistic
+ baseline were thorough
+ simple and effective

error on creating the 2-D representation regarding object pose, shape, and type.
It is indicated that no prior knowledge is assumed about the objects
raw image from the in-hand camera is used to infer all of this information to create the 2-D representation

Does it ever output the wrong shape? 
small ... it matter even if it were wrong?
see scenes with very differently sized objects, and not just primitive shapes

extended to truly 3-D environments
go up or down relative to the table
The observability representations used are strictly 2-D
2 shelves, one target
genuine pile of objects
How will you scale your method to these (more realistic) scenarios? It’d be great to discuss in the paper.

video: at least one of the baselines is shown also

I think performance will definitely degrade as noisy real images are not going to produce as clean of representations as can be achieved in simulation. 

+ But the core ideas of the algorithm set the stage for applying it in these more complicated settings.

---------------------------------------------------------------------------------
---------------------------------------------------------------------------------

- it is essentially planar

- Observations for the system aren’t noisy, beyond the fact that if an object is not 50\% visible, it is not considered.

- Does the algorithm take care of toppling displaced objects?
  trained in a 2D How realistic is that? stacking, object shapes vary with height. 
  dynamics as flat or high objects will behave differently
  
- high clutter picking non-target objects might be totally unavoidable

- objects very simple. generalize to more real/complex shapes? Adding those in testing to see performance would help.

- introduction = related work section, without highlighting, explaining or motivating the proposed approach until the very end.

- Before related work, make more clear what is the problem and approach proposed. 
  For instance, it isn’t clear that this paper cares about not dropping objects from a shelf until section 3.

- During intro RHP are assumed known, add short explanation.

- In line 107, “We do not assume any prior knowledge on the number, pose, and shape of the objects on the shelf.”  
  Object shape in training affect the results. extremely simple, suffer: real with diverse shapes and textures.

- cannot perform well with scenes that have many more than 10 objects, as these scenarios do not appear in training and are also not tested.

- Line 109 “single optimization problem with the objective of minimizing the total number of actions.”,  
  doing nothing would be the best policy.
  
- How is the “type” of an object described? Specially if there is now prior knowledge on the shapes or objects, how can the algorithm reason over that?

- Line 125 is not obvious “we opt for a uniform negative reward per action, casting the problem as a stochastic shortest path”. What is “uniform negative reward”? Does uniform here refer to a uniform distribution or just a constant? What is the implication of it being a stochastic shortest path?
    Response: A stochastic shortest-path problem(sspp) hS, A, T, C, Gi is an mdp in which all
    rewards are negative  (See definition 2 in ``Integrated task and motion planning in belief space'')
            
- Fig. 3 is rather simple and not enough to understand the complete approach. For instance, the role of previous observations is missing, or how RHP is used.

- Line 150, how is it possible to represent objects in an image if no prior knowledge of the shape is known (as said in line 107)? An image obtained from the in-hand camera would not be able to provide shape information beyond the pixels it can capture. However, the example observation in Fig 3. does show knowledge of the full geometry of the objects. It is unclear how task prior can help on that without really knowing having access to prior knowledge on the objects. Even the accumulation of observations woulndt be enough to tell what is the shape of an object at the back of the shelf.
  Response: Agree, shapes should be moved to task priors.

- The generated raw images are noise free which makes them unrealistic to render in a real scenario. Especially if again there is no prior knowledge on object shapes, real depth images will be noisy and correcting for that without prior shape information seems difficult.

- The paper relies on access to a simulator from which it is possible to render the effect of the actions taken during RHP. However, in a real scenario, this simulator and rendered images are unlikely to be accurate, which could largely hurt the approach.

- How does the algorithm account from objects falling from the shelf? Is it just by having a sparse reward like the one that marks zero if an object fails or the target is not reached, and 1 otherwise?

- Line 234, what does “data point” refer to in this sentence?

- Line 253, the greedy baseline is unclear. Why is the mean of the action a good idea? Why is this helping to understand the value of predicting target pose distribution?

- I would make sense to have a baseline that takes the most likely target pose and performs the predicted action for that pose.
 Response: Will do so

- Line 282, could you clarify this: “vertices around the object’s centre within 0.1 cm and 5.0 cm in range.”?

- In line 289, what does it mean “with all its parametrizations”?

- In the realistic experiments, the set of observations is still rendered as in the training/2D planar case? What objects are used? Same as in the 2D case?

- Video: It would be nice to include something that represent which action was selected. maybe an arrow for motion and something different when gripper is closing.

- RW: There is much more complexity in the real world than just different physics parameters.


==> icra_rev.tex <==
training the three-headed NN:
    1) this type of loss has existed out there, such as in the work [Kei Kase, etc. Transferable Task Execution from Pixels through Deep Planning Domain Learning, ICRA2020]; 
    2) Using RNN to perform implicit belief updating has also been widely used in RL community.

RHP: planning is actually an evaluation for the learned policy

The planning is then not motivated well, why not just run the learned policy? 

Without the supervised loss, the policy may not learn good reasoning about the target object pose distribution. 

RHP planning is a biased approximation to the learned policy

It is not clear about how the target object’s position is sampled in the testing, which actually also affects all methods’ performance, especially to the biased RHP planner.

more than 10 (maximum in training)

If the target object is changed, or the target objects are very different in shape

this work requests the objects with the same height and the robot movements in the 2D space
 
it is not clear how each object’s polygon-shape is
sampled during the training

---------------------------------------------------------------
---------------------------------------------------------------

but is not preferable when it comes to time spent

assumptions/inputs to the approach would be more clearly stated

How is the search query represented?

(given multiple objects of the same “type” exist in the shelf)	Would this just be outsourced as a new “type”?

This will require an externally calibrated camera sensor.

The abstract image-based representation is world-instead of ego-centric. Have you experimented with an ego-centric representation 

it would also help if NN/V/pi would be written as an input.

p. 2: “Since the state of is not always accessible”

----------------------------------------------------------------
----------------------------------------------------------------
what exactly is the observation space?  
Is the (simulated) camera RGB only, or does it contain depth?  
What exactly is the action space?  
How is the library of object type-shape pairs represented, 
and how does the system know which object is the target?
- A framework for push-grasping in clutter.  Mehmet R. Dogar and Siddhartha S. Srinivasa, RSS 2011.
- Robot Grasping in Clutter: Using a Hierarchy of Supervisors for Learning from Demonstrations.  Michael Laskey, Jonathan Lee, Caleb Chuck, David Gealy, Wesley Hsieh, Florian T. Pokorny, Anca D. Dragan, and Ken Goldberg, CASE 2016.

p2:  "approaches sated so far"
p2:  "the state of is not always"
p5, Alg 3.  "end" before "else"
p4. Alg 1.  Wouldn't it be simpler (and equivalent) to just
store the best action so far?
p4, Alg 2.  After $R \gets R ...$, what is $^1 r$?
Ref [14,34] errors
Video at 0:14  "eperiements"

==> iros_rev.tex <==
REV 18405 : ++
1) (reality gap): Added sentence to Introduction Section, RHP paragraph + added reference to PhD thesis for more details
2) (action space definition): Introduction Section, Assumptions paragraph (last)
3) (clarification on performance): DONE


REV 18413 : +
1. The occlusion in test scene is simple, the performance
of the algorithm in more clutter scenes needs to be
verified.
2. This paper is well-writing except the planner part,
which is hard to understand.
3. It is a pity that there is no follow-up discussion on
the failure cases caused by corners,I think that a new type
of interaction can be introduced to solve it. 

REV 20761: +
1)  2D planar actions is a strong limitation 
2) Why A2C not SAC
3) Compare with baseline [27]
4) RL learning details

REV 21157: --
1) LSTM: length of the sequence
2) Having a look at the video which includes both the real
scene and simulation environment, it is not clear how the
green object appears in the simulation even though it is
not yet seen in the real setting. Since it is mentioned
that the generative head for object pose is trained in a
supervised manner, how is it labelled while executing the
RHP in test time.
3) training details
4) how is the position of the object
extracted from the pixel intensities?

==> meta_reviews.tex <==
3. Please summarize your comments. (Visible to author after author notification)
This paper addresses the problem of finding a known target object in clutter through physical rearrangement of objects. The paper presents a hybrid model-based, model-free approach for performing this operation in an explicit POMDP model of the task.

All reviewers acknowledge the importance and difficulty of the target task.

Reviewer #2 finds the method to be essentially a combination of existing techniques designed for this task, while reviewer #3 finds the presentation too unclear to articulate exactly what the novelty of the method is over existing work.

The reviewers bring up significant concerns about the complexity of the environment, namely that all objects have the same height and similar shape, greatly simplifying the problem. This is further complicated by no simulated camera noise in the experiments making them far from reality. While the reviewers bring up the scenario of grocery shelves as a possible place where the shape and height assumptions are valid, this is a much more specific application than those claimed in the paper and still suffers from the need to deal with highly variable object appearance and materials such as metal cans or transparent containers that can be IR absorbent rendering depth cameras difficult to use without significant processing.

All reviewers also note that the paper's claims of requiring no prior knowledge of the objects is misleading, as at least knowledge of the class of object shape primitives is present in design of the algorithm / learning.

Furthermore, the highly idealized simulation examples are rendered much weaker in the context of related work on actual physical systems with variable object shapes such as the "Mechanical Search" work from Goldberg's lab which is not cited in the submitted paper (see http://ai.stanford.edu/mech-search/)

As such I recommend rejection of the paper.

==> notes.tex <==
%#############################
%#############################
TODO (after submission!)
expected sum of the \emph{return} --> expected \emph{return}  VVVVV
$\Bar{o}_i$.append$(o)$ update its location in algo    VVVV
the advantage should have r_i in it    VVVVVV
use $\mathcal{O}^i$ in hierarchical rearrange and retrieve  VVVV
The stochastic and greedy policIES exhibit similar   VVVVV
We use $m$=$4$ and $h$=$4$ as THEY OFFER a reasonable balance VVVVV
Examples of tasks solved with the hybrid planner are SHOWN in VVVV
and in the attached video --> in the experiments' video    -------
connecting state to observation is  the observation probability distribution $\Omega : S \times O \rightarrow [0,1]$  -------
long action sequences becomes impractical REMOVE S from become VVVVV
Since the state of is not always IN METHODOLOGY
They tackle top-down bin decluttering by removing obstructings
%#############################
%#############################

ICRA
why 2D is useful and important
shape variance (figures to show noise)

Add a brief description of RHP in the Introduction
Make the introduction sound less like Related Work
Clearly state the contribution of the work relative to previous work
Make the tracking the distribution over the target object pose more central

ADD: state dimention is variable, number of object is not known a priori.
RL IL
%#############################
%#############################
meta reviews:
- novelty is unclear, combination of existing work
- complexity of the environment, object shape, camera noise
- object appearance and materials such as metal cans or transparent containers are hard to detect
- no prior knowledge? at least knowledge of the class of object shape primitives is present!
- highly idealized simulation examples

%#############################
%#############################
Rev3: (I don't understand what he understood from our approach)

- If the state vector is of variable size, how does the RL algorithm deal with that? 
- The RHP seems to have access to a physics simulator. That makes the statement also weird. Being able to simulate the environment offline to do (heuristic)planning means there is full god-like knowledge of the whole scene.

- why not go completely model-free (ans: it is a baseline)

- object seems to be disappearing between frames (ans: if more than 50/100 is occluded, then they are not detectable and hence disappear) 

- task priors? (ans: the explanation is clear in the text and in the figure!)

- How good is the policy after Imitation learning? How good is the pose-estimator? (ans: add IL baseline? but this has been adressed in previous work)

- Sharing parameters is not about the "significance" it is about having "Compatible Features" representations between the policy and value function, return to Sutton for more details.
%#############################

==> plots_two_col.tex <==
\begin{figure*}[t]
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{sr_objNb}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=11, ymin=50, ymax=100,
    ylabel={Success rate \%}, xlabel={Number of obstacles}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0.0,-0.5)},anchor=south west,legend columns=7, draw=none, opacity=0.0, font=\scriptsize},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]     table[x index=0,y =hyb6,col sep=comma]   {sr_0.dat};
 	\addplot [blue,          line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]      table[x index=0,y =hyb4,col sep=comma]   {sr_0.dat};
 	\addplot [blue!50!white, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb2,col sep=comma]   {sr_0.dat};
 	\addplot [orange!90!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {sr_0.dat};
  	\addplot [red!70!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {sr_0.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {sr_0.dat};
 	\addplot [green!60!black, line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]   table[x index=0,y =sto,col sep=comma]    {sr_0.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {sr_0.dat}; 
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy60) at (axis cs:0,60) {};
	\node (sy70) at (axis cs:0,70) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy90) at (axis cs:0,90) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:10,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy70) -- (ex |- sy70);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy90) -- (ex |- sy90);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{t_objNb}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=11, ymin=0, ymax=100,
    ylabel={Time in seconds}, xlabel={Number of obstacles}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize, 
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb6,col sep=comma]   {t_0.dat};
 	\addplot [blue,           line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb4,col sep=comma]   {t_0.dat};
 	\addplot [blue!50!white,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb2,col sep=comma]   {t_0.dat};
 	\addplot [orange!90!black,line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {t_0.dat};
  	\addplot [red!70!black,   line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {t_0.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {t_0.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid, scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {t_0.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {t_0.dat}; 
% 	\addlegendimage{empty legend}
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy20) at (axis cs:0,20) {};
	\node (sy40) at (axis cs:0,40) {};
    \node (sy60) at (axis cs:0,60) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:10,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy40) -- (ex |- sy40);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{ac_objNb}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=11, ymin=0, ymax=35,
    ylabel={Number of actions}, xlabel={Number of obstacles}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize,
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb6,col sep=comma]   {ac_0.dat};
 	\addplot [blue,           line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb4,col sep=comma]   {ac_0.dat};
 	\addplot [blue!50!white,  line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]              table[x index=0,y =hyb2,col sep=comma]   {ac_0.dat};
 	\addplot [orange!90!black,line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {ac_0.dat};
  	\addplot [red!70!black,   line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {ac_0.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {ac_0.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {ac_0.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {ac_0.dat}; 
 	\legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy5) at (axis cs:0,5) {};
	\node (sy10) at (axis cs:0,10) {};
    \node (sy15) at (axis cs:0,15) {};
    \node (sy20) at (axis cs:0,20) {};
    \node (sy25) at (axis cs:0,25) {};
    \node (sy30) at (axis cs:0,30) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:10,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy5) -- (ex |- sy5);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy10) -- (ex |- sy10);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy15) -- (ex |- sy15);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy25) -- (ex |- sy25);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy30) -- (ex |- sy30);
\end{tikzpicture}
% \vspace{-20pt}
\end{minipage}
% \caption{Performance \wrt clutter density.}
% \label{exp:clutterDense}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
% [-1ex] 
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{sr_noisy}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=0.25, ymin=50, ymax=100,
    ylabel={Success rate \%}, xlabel={noise levels}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]   table[x index=0,y =hyb6,col sep=comma] {sr_n.dat};
 	\addplot [blue, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]            table[x index=0,y =hyb4,col sep=comma] {sr_n.dat};
 	\addplot [blue!50!white,   line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]   table[x index=0,y =hyb2,col sep=comma] {sr_n.dat};
 	\addplot [orange!90!black, line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]  table[x index=0,y =hyb4_lim,col sep=comma] {sr_n.dat};
  	\addplot [red!70!black,    line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]  table[x index=0,y =gre, col sep=comma] {sr_n.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]  table[x index=0,y =gre_hm,col sep=comma] {sr_n.dat};
 	\addplot [green!60!black, line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]  table[x index=0,y =sto, col sep=comma] {sr_n.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}] table[x index=0,y =mod, col sep=comma] {sr_n.dat}; 
    % \legend{Greedy, Greedy$_{gen}$, Stochastic, Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hierarchical}
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy60) at (axis cs:0,60) {};
	\node (sy70) at (axis cs:0,70) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy90) at (axis cs:0,90) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:0.25,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy70) -- (ex |- sy70);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy90) -- (ex |- sy90);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}
% \vspace{-8pt}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{t_noisy}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=0.25, ymin=0, ymax=100,
    ylabel={Time in seconds}, xlabel={noise levels}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize, 
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb6,col sep=comma]   {t_n.dat};
 	\addplot [blue,          line width=0.8pt, mark=diamond*, mark options={solid},scale=0.8]    table[x index=0,y =hyb4,col sep=comma]   {t_n.dat};
 	\addplot [blue!50!white, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb2,col sep=comma]   {t_n.dat};
 	\addplot [orange!90!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {t_n.dat};
  	\addplot [red!70!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {t_n.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {t_n.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {t_n.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {t_n.dat}; 
    % \legend{Greedy, Greedy$_{gen}$, Stochastic, Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hierarchical}
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\addlegendimage{empty legend}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy20) at (axis cs:0,20) {};
	\node (sy40) at (axis cs:0,40) {};
    \node (sy60) at (axis cs:0,60) {};
    \node (sy80) at (axis cs:0,80) {};
    \node (sy100) at (axis cs:0,100) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:0.25,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy40) -- (ex |- sy40);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy60) -- (ex |- sy60);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy80) -- (ex |- sy80);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy100) -- (ex |- sy100);
\end{tikzpicture}
\end{minipage}%
% \vspace{-8pt}
\hfill
\begin{minipage}{0.3\textwidth}
\centering
\tikzsetnextfilename{ac_noisy}
\begin{tikzpicture}
	\begin{axis}[
    x post scale=0.5, y post scale=0.3,
    xmin=0, xmax=0.25, ymin=0, ymax=35,
    ylabel={Number of actions}, xlabel={noise levels}, 
    axis x line*=bottom,  axis y line*=left,
    label style={font=\scriptsize}, tick label style={font=\scriptsize},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},anchor=south},
    legend style={at={(0,-0.7)},anchor=south west,legend columns=7, font=\scriptsize,
    draw=none, opacity=0.0},
    legend cell align={left}, % The command for legend alignment
	]
 	\addplot [blue!50!black, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb6,col sep=comma]   {ac_n.dat};
 	\addplot [blue,          line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb4,col sep=comma]   {ac_n.dat};
 	\addplot [blue!50!white, line width=0.8pt, mark=diamond*, mark options={solid,scale=0.8}]    table[x index=0,y =hyb2,col sep=comma]   {ac_n.dat};
 	\addplot [orange!90!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =hyb4_lim,col sep=comma] {ac_n.dat};
  	\addplot [red!70!black,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre,col sep=comma]    {ac_n.dat};
%   	\addplot [red!60!white,  line width=0.8pt, mark=square*,  mark options={solid, scale=0.5}]   table[x index=0,y =gre_hm,col sep=comma] {ac_n.dat};
 	\addplot [green!60!black,line width=0.8pt, mark=*,        mark options={solid,scale=0.5}]    table[x index=0,y =sto,col sep=comma]    {ac_n.dat};
 	\addplot [black,line width=0.8pt, mark=triangle*,mark options={solid,rotate=118,scale=0.6}]  table[x index=0,y =mod,col sep=comma]    {ac_n.dat}; 
    \legend{Hybrid$_{6\times6}$, Hybrid$_{4\times4}$, Hybrid$_{2\times2}$, Hybrid$_{4\times4}^{\textrm{lim}}$, Greedy, Stochastic, Hierarchical}
	\node (sy00) at (axis cs:0,00) {};
	\node (sy5) at (axis cs:0,5) {};
	\node (sy10) at (axis cs:0,10) {};
    \node (sy15) at (axis cs:0,15) {};
    \node (sy20) at (axis cs:0,20) {};
    \node (sy25) at (axis cs:0,25) {};
    \node (sy30) at (axis cs:0,30) {};
	\node (sx) at (0,100) {};
	\node (ex) at (axis cs:0.25,100) {};
	\end{axis}
	\draw [thin, dashed, draw opacity=0.1] (sx |- sy00) -- (ex |- sy00);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy5) -- (ex |- sy5);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy10) -- (ex |- sy10);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy15) -- (ex |- sy15);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy20) -- (ex |- sy20);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy25) -- (ex |- sy25);
	\draw [thin, dashed, draw opacity=0.2] (sx |- sy30) -- (ex |- sy30);
\end{tikzpicture}
\end{minipage}
\caption{Performance \wrt different clutter densities and noise levels.}
\label{exp:sim}
\end{figure*}

==> response.tex <==
We would like to thank the reviewers for their thorough analysis, and address the main questions raised. 

- R1 “It is indicated that no prior knowledge is assumed about the objects […] The 2-D representations shown in the figures [...] look very clean to me.” R2 “how is it possible to represent objects in an image if no prior knowledge of the shape is known (as said in line 107)?”  

We apologize for the confusion on object shapes. When we indicated that no prior knowledge is assumed about the objects, we should have clarified that it only refers to the neural network (NN), which is trained with randomized arbitrary shapes. However, during execution, the overall system is given a library of object types and shapes. Object recognition on the present scene detects poses and types. This allows the system to place the correct shape (however complex) in the intermediate abstract representation. This abstract representation is then fed into the NN. 

- R1 “Does it ever output the wrong shape?” “It will be more compelling to see scenes with very differently sized objects.” R2 “How can this approach generalize to more real/complex shapes?” 

Object shape at execution time doesn’t need to exactly match object shape during training. We should have clarified that we do inject noise in the objects’ shape in the experiments of Fig. 6. This is what we meant by “vertices around the object’s centre within 0.1 cm and 5.0 cm in range” (which R2 asked us to clarify). To add noise onto the shapes, each vertex of an object gets a new coordinate in the object frame at every action step. The new coordinate is sampled from a Gaussian distribution centered at the initial coordinate of that vertex. By changing the Gaussian standard deviation from 0.05 (low noise) to 0.25 (high noise), we observed variation in the vertex coordinate anywhere between 0.1 cm and 5.0 cm w.r.t. to its initial location (in this experiment circles are replaced with octagons). For example, under high noise, an octagon object will have a very arbitrary shape.  

- R1 “It would be helpful to include some discussion about how this could be extended to truly 3-D environments.” R2 “The approach is trained in a 2D scenario, and even in Mujoco, the scenes are practically planar. How realistic is that?” 

We acknowledge that currently the approach solves 2D problems. However, we note that (i) planning under partial observability is a significant challenge in such multi-object environments, even in 2D; (ii) there are some practical problems, particularly shelves with limited height e.g. in supermarket shelves, where the current 2D planner can be immediately useful; (iii) our work is novel in proposing to learn to predict the possible locations of the hidden object, to deal with the partial observability, which we think is a useful contribution to solving this important problem; (iv) this idea of learning to predict the belief state seems applicable to 3D as well, e.g. using colour-labelled voxelated representations for the space and objects, which we leave as future work.  We also note that there were some admittedly limited 3D features of our system. Our realistic experiments were conducted in a 3D simulator, where the length of the shadow behind each object is affected by the relative height of the in-hand camera to the top of the objects.   

R2:  

- “It would make sense to have a baseline that takes the most likely target pose and performs the predicted action for that pose”  

We indeed experimented with this method during the development of this work. We don’t think it is a “baseline”, in the sense that it is still using the NN predictions about the hidden object location, and therefore is a variation of our method. The experiments showed that this variation achieved a slightly lower success rate, and therefore, in the paper, we used the proposed weighting scheme. We also note that, on average, our system generates 1.3 potential positions for the target object, and therefore the resulting planning and execution time are quite similar in practice. 

- “the distribution of training shapes for instance will clearly affect the results at test time. [...] Same with number of objects, there is no reason to believe that this approach can perform well with scenes that have many more than 10 objects”  

We agree that the distribution used in training must be somewhat representative of the shapes the system will see during execution. This is unavoidable in machine learning. However, the approach, in principle, is not limited to certain shapes or a predefined number of objects, thanks to the generalization provided by the training of the CNN. 

- “What is “uniform negative reward”?”, “How does the algorithm account from objects falling from the shelf?”  

We apologize this was unclear. By “uniform”, in this context we indeed mean constant. That is, we do not design more articulated reward functions that encode hints of what we think is the solution (as in reward shaping). Consequently, each no-terminal action has the same negative cost, and the problem is therefore a shortest-path problem. When an object, during training, falls off the shelf, the episode ends with an additional large negative reward.  

- “However, in a real scenario, this simulator and rendered images are unlikely to be accurate, which could largely hurt the approach.”  

This is a crucial aspect of our approach. The use of the learned policy and value function allows the planner to work on a short horizon, which allows fast MPC-like replanning at every time step.  Thus, we minimize compounding errors due to such inaccuracies (e.g. simulator or object detection inaccuracies). The abstract representation is updated at every iteration. 

- “Line 234, what does “data point” refer to” 

 It refers to the data points of the experiments’ plots in Fig. 6. 

- “If there is enough clutter and environment constraints, picking non-target objects might be totally unavoidable in order to retrieve a target goal.”  

The system can indeed learn to perform actions that are like two-fingered gripping, to move objects out of the way, as shown in Task 4 in the video. 

- “In the realistic experiments, the set of observations is still rendered as in the training/2D planar case? What objects are used? Same as in the 2D case?”  

In the realistic experiments, we used 3D boxes and cylinders. They had different dimensions from the objects used during training. 

- “Line 253, the greedy baseline is unclear. Why is the mean of the action a good idea?” 

The policy is represented as a Gaussian by the NN. Picking the mean of this Gaussian gives us the most likely action that maximizes the expected return, according to the network.  

- “Why is this helping to understand the value of predicting target pose distribution?” 

We wanted to see if training the network to predict the target pose distribution would create a latent representation that also helps with learning a better policy. 

==> reviews.tex <==
3. Please summarize the paper, state what you think the contribution is, comment on its strengths and weaknesses, and give advice for improving the paper.
The paper provides a hybrid model-free/model-based approach to doing object retrieval in partially observed cluttered table-top environments, both 2-D and 3-D. The model-based component is a receding horizon planner (i.e. model predictive control scheme) that takes an initial environment state and uses a physics simulator to execute actions generated by a stochastic policy previously learned in a model-free RL fashion in simulation. The model-free component predicts the initial state that the model-based component is initialized with. The state representation is specific to this table-top manipulation setting and is a 2-D abstract image showing the shapes and poses of objects (both a target object to be grasped and the other objects causing clutter), the boundaries of the environment, and importantly for this partially observed setting, different colorings for regions that are known to be free space and regions that have not been observed yet. This is an extension of previous work that assumed fully observable scenes. This abstraction is learned with a neural network from raw RGB image observations, where an LSTM recurrent neural network is used for the policy/value function learning to accommodate a history of observations and cope with the partial observability. There is also an image generator output head that produces a kernel density estimate of where the target object to be grasped is located in the scene. This heuristically guides the action selection. The policy learning is based on a curriculum such that it starts learning with a small number of objects and works its way up to ~10 objects in the scene causing significant clutter.

The paper is very clearly written. I like the abstract representation that is generated from observations, particularly that it explicitly differentiates between regions it has observed to be free space and regions that it has not yet observed due to occlusions. While the representation is perhaps optimized for this specific setting of table-top manipulation and the environments are simplistic, I think demonstrating its efficacy even in this simple environment is a good contribution, and the baseline algorithms in the experiments were thorough enough to show the proposed hybrid planner is successful. This to me seems like a relatively simple and effective way to handle partial observability for these environments. I advocate for acceptance and give some minor feedback as follows to improve the paper.

I would be interested to see more information about the error on creating the 2-D representation (especially from the 3-D environment) regarding object pose, shape, and type. It is indicated that no prior knowledge is assumed about the objects and the raw image from the in-hand camera is used to infer all of this information to create the 2-D representation. The 2-D representations shown in the figures and video look very clean to me. I could see though how there could be ambiguity working just from RGB images, especially if low-resolution images are input to the network, e.g. a cylinder from a low-profile straight-on view can look like a box. Does it ever output the wrong shape? And since the objects appear to all have similar dimensions, would it matter even if it were wrong? I think it will be more compelling to see scenes with very differently sized objects, and not just primitive shapes but more complicated object meshes that you would find in the real world.

It would be helpful to include some discussion about how this could be extended to truly 3-D environments. I realize a 3-D simulator is used in the experiments, but the objects are all located on a planar surface and the objects are all the same height. Also the robots actions are effectively in the plane, it does not go up or down relative to the table. The observability representations used are strictly 2-D. How will you extend to 3-D if you now have say a bookshelf with 2 shelves, and there is clutter on both levels but still just one target object to find. Or if the clutter is not so singulated and you have a genuine pile of objects to sift through. This presumably also complicates the action space more as there will be many more possibilities to be explored. How will you scale your method to these (more realistic) scenarios? It’d be great to discuss in the paper.

Small corrections:
Pg. 1, Paragraph 1: “Autonomously manipulating everyday objects…”
Pg. 5, 7.1, “... and none of the objects are dropped…”
Is the batch size correct? It’s reported in experiments Section 7.2 that batch size is 15,000. That seems quite large for image-based data

------------------------------------------------------------
POST REBUTTAL
Thank you to the authors for addressing our concerns. In view of the rebuttal comments and discussions with reviewers, I think the method is a nice extension of citation [14] to operate in partially observable tabletop environments where a top-down view is not possible and object models are not known. The biggest improvement to the paper would be to have experiments with real object meshes (e.g. objects from YCB dataset). In this case the primitive shape approximations will impose more error in the representation relative to the real world. Also doing this with a more realistic camera model and lighting conditions (preferably doing the experiments on a real platform) would be more compelling.

It should also be clarified in the paper about what prior information is used in training and execution. Specifically, discuss further the library of primitives being used. It is misleading to say "no prior information" was used as having candidate primitive shapes in training or to choose from at execution is a shape prior. Probably better to say known object models are not required, and are approximated with shape primitives. The real mesh experiments would then validate whether this approximation is okay in this setting.
4. Was the video submission useful? What was good about it? What could be done to improve it? (Write N/A if there was no video submission)
The video was good in that it showed the core task being performed, and I especially liked that it showed what the planner was reasoning over at every timestep, and how the observation representation was evolving. It's nice that multiple executions are shown, but they are not qualitatively very different so I felt it was a bit redundant watching the entire video. It would be more helpful to show one execution where at least one of the baselines is shown also, especially if there are interesting qualitative differences in the baselines that fail compared to the hybrid planner.
5. If code was submitted, we ask that you perform a sanity check. We do not ask that you run the code. But if you do, please comment on this too. Authors have been instructed to provide a readme file that points to the part of the code that needs to be peer-reviewed. Please, read this part of the code and answer the following questions: a) Does the code appear to implement the algorithm described in the paper? b) Did the readme file allow you to identify relevant parts of the code? c) Were you provided with data to replicate the results? Please, remember that code is for peer-review only and that you are not allowed to use this code outside the review process. (Write N/A if there was no code submission)
N/A
9. Comment on the potential impact of the paper to real robotics problems (taking COVID-19 impact into account). Please check the supplement material for the COVID-19 response.
I do not doubt that this method would work in the real world, though I think performance will definitely degrade as noisy real images are not going to produce as clean of representations as can be achieved in simulation. Surely manipulation in clutter and partial observability is crucial for real world manipulation. I think the task as performed in the experiments is perhaps a little contrived, one would expect more object size variability and a less uniform distribution of objects in e.g. a kitchen cupboard. But the core ideas of the algorithm set the stage for applying it in these more complicated settings.
12. Overall recommendation:
Weak Accept
13. Rate your level of confidence in this recommendation:
High
Reviewer #2
Questions
3. Please summarize the paper, state what you think the contribution is, comment on its strengths and weaknesses, and give advice for improving the paper.
A . Paper summary and contributions

This paper aims at solving the problem of picking a target object from a shelf, in a mostly planar setting, without dropping objects from the shelf.

It contributes by:
(i) Proposing a hybrid planner that first predicts a pose distribution of the target objects as well as, policy values and actions.
(ii) The most likely poses are then evaluated using RHP. The resulting best policy value when weighted by the likelihood of each pose is executed in an MPC fashion.

The approach is only tested in simulation, it is essentially planar, and the shape of the objects is reduced to circles, squares and triangles. Observations for the system aren’t noisy, beyond the fact that if an object is not 50% visible, it is not considered.

B . Positive aspects of the paper

The paper acknowledges the importance of dealing with cluttered environments where noise and uncertainty can arise in several dimensions including motion of objects or observations with limited information on the state.
The paper evaluates the approach on a different simulator and is capable of producing a performance of 88% in a novel simulator.

C. Feedback on the paper

Does the algorithm take care of toppling displaced objects?

The approach is trained in a 2D scenario, and even in Mujoco, the scenes are practically planar. How realistic is that? In many cluttered environments, stacking is quite common. Or simply, object shapes vary with height which is not contemplated in this work. Moreover, the simplification of 2D can cause further problems when learning the dynamics as flat or high objects will behave differently under pushing actions for instance.


If there is enough clutter and environment constraints, picking non-target objects might be totally unavoidable in order to retrieve a target goal. However this paper seems unable to deal with such scenarios.

The objects considered are far from realistic and very simple. I only observed cylinder-like rectangles, circles and triangles. How can this approach generalize to more real/complex shapes? Adding those in testing to see performance would help.

On the introduction, right now it reads more like a related work section, without highlighting, explaining or motivating the proposed approach until the very end.

Before going into the related work, it would suggest to make more clear what is the problem and approach proposed. Otherwise it is hard to follow the reasoning behind the structure and content of the related work. For instance, it isn’t clear that this paper cares about not dropping objects from a shelf until section 3.

During intro and related work, RHP are assumed known, however I would expect that many readers would benefit from a short explanation.


In line 107, “We do not assume any prior knowledge on the number, pose, and shape of the objects on the shelf.” However the distribution of training shapes for instance will clearly affect the results at test time. Specially when the objects considered are extremely simple, this is likely to suffer when objects are more real with diverse shapes and textures. Same with number of objects, there is no reason to believe that this approach can perform well with scenes that have many more than 10 objects, as these scenarios do not appear in training and are also not tested.

Line 109 says that “single optimization problem with the objective of minimizing the total number of actions.”, however this should mention that the actual goal is to retrieve a target, not just perform a minimum number of actions, where doing nothing would be the best policy.

How is the “type” of an object described? Specially if there is now prior knowledge on the shapes or objects, how can the algorithm reason over that?

Line 125 is not obvious “we opt for a uniform negative reward per action, casting the problem as a stochastic shortest path”. What is “uniform negative reward”? Does uniform here refer to a uniform distribution or just a constant? What is the implication of it being a stochastic shortest path?

Fig. 3 is rather simple and not enough to understand the complete approach. For instance, the role of previous observations is missing, or how RHP is used.

Line 150, how is it possible to represent objects in an image if no prior knowledge of the shape is known (as said in line 107)? An image obtained from the in-hand camera would not be able to provide shape information beyond the pixels it can capture. However, the example observation in Fig 3. does show knowledge of the full geometry of the objects. It is unclear how task prior can help on that without really knowing having access to prior knowledge on the objects. Even the accumulation of observations woulndt be enough to tell what is the shape of an object at the back of the shelf.

The generated raw images are noise free which makes them unrealistic to render in a real scenario. Especially if again there is no prior knowledge on object shapes, real depth images will be noisy and correcting for that without prior shape information seems difficult.

The paper relies on access to a simulator from which it is possible to render the effect of the actions taken during RHP. However, in a real scenario, this simulator and rendered images are unlikely to be accurate, which could largely hurt the approach.

How does the algorithm account from objects falling from the shelf? Is it just by having a sparse reward like the one that marks zero if an object fails or the target is not reached, and 1 otherwise?

Line 234, what does “data point” refer to in this sentence?

Line 253, the greedy baseline is unclear. Why is the mean of the action a good idea? Why is this helping to understand the value of predicting target pose distribution?

I would make sense to have a baseline that takes the most likely target pose and performs the predicted action for that pose.

Line 282, could you clarify this: “vertices around the object’s centre within 0.1 cm and 5.0 cm in range.”?

In line 289, what does it mean “with all its parametrizations”?

In the realistic experiments, the set of observations is still rendered as in the training/2D planar case? What objects are used? Same as in the 2D case?

The paper would benefit from discussing what are the main failure cases of their approach. What happens in that 10% of cases that can’t be solved.
4. Was the video submission useful? What was good about it? What could be done to improve it? (Write N/A if there was no video submission)
The video is useful, and quite easy to follow even before reading the paper. It would be nice to include something that represent which action was selected. maybe an arrow for motion and something different when gripper is closing.
5. If code was submitted, we ask that you perform a sanity check. We do not ask that you run the code. But if you do, please comment on this too. Authors have been instructed to provide a readme file that points to the part of the code that needs to be peer-reviewed. Please, read this part of the code and answer the following questions: a) Does the code appear to implement the algorithm described in the paper? b) Did the readme file allow you to identify relevant parts of the code? c) Were you provided with data to replicate the results? Please, remember that code is for peer-review only and that you are not allowed to use this code outside the review process. (Write N/A if there was no code submission)
N/A
9. Comment on the potential impact of the paper to real robotics problems (taking COVID-19 impact into account). Please check the supplement material for the COVID-19 response.
I believe this paper is not ready to be implemented in a real robotic platform and achieve the same level of performance.
While the authors say: "To our approach, the real world would be just another execution environment which we do not know its exact physics parameters.” There is much more complexity in the real world than just different physics parameters.
Real image observations are much more noise, and object shapes are more complex than the tested ones. Moreover, assuming planar scenarios is not realistic as objects have different height and vertical shapes which changes their dynamics.
12. Overall recommendation:
Weak Reject
13. Rate your level of confidence in this recommendation:
High
Reviewer #3
Questions
3. Please summarize the paper, state what you think the contribution is, comment on its strengths and weaknesses, and give advice for improving the paper.
The paper proposes a hybrid-scheme of model-free RL and heuristic-based planning for learning to act in a partially observable and visually cluttered environment in order to find and retrieve certain target objects. This combination is done in the spirit of Play Online Learn Offline (POLO) [14], albeit by replacing the trajectory optimization part with a heuristic-based search. The paper presents benchmarks on a simulated setup and compares it to a few baseline variants.

# Strengths:
----------------
* The paper attempts to solve a hard problem in general and does so while relying on visual input. The results while limited do show a working algorithm. The paper brings together different concepts from state-of-the-art to solve a significant challenge in robotics.

# Weakness:
-----------------
* The paper seems to gloss over many important details in my opinion. The presentation is often not clear. Some parts are very text-verbose and still somewhat confusing. As a suggestion, consider drawing a simple schematic to simplify the description of how all these moving parts come together. Another way is to introduce a bit more structure and divide the presentation of the algorithm to multiple smaller problems.

# Major Comments:
--------------------------
The following points follow no clear order of importance.

* The paper mentions that no priors about the number of objects or their shapes and poses. This claim raises two points:
1)- Is the state vector of variable size, since it contains some parameters from every object in the scene and some might be occluded in the beginning. If the state vector is of variable size, how does the RL algorithm deal with that? That seems like a non-standard RL setting. If not then this statement is somewhat misleading.

2)- The RHP seems to have access to a physics simulator. That makes the statement also weird. Being able to simulate the environment offline to do (heuristic)planning means there is full god-like knowledge of the whole scene.

* What is meant by task priors? I don't think this term has been clearly defined anywhere in the paper.

* I think it is crucial to be able to see the learning performance of the pose-estimator in order to provide a sanity-check for this part of the approach. Also, some testing of how this estimator may generalize would be great. In the video, the target object seems to be disappearing between frames while planning, I am not sure what that is a sign of.

* Sharing parameters is not about the "significance" it is about having "Compatible Features" representations between the policy and value function, return to Sutton for more details.

* Another significant point is the role of Imitation Learning. How good is the policy after Imitation learning? How good is the pose-estimator? It is important to show this baseline, in order to make the point that the RL/planning is actually improving something. Also, 10000 Samples of imitation pairs sound like a lot when considering that this has to be executed on a real robot. It would be interesting to see how the performance scales with the number of demonstrations and with their absence.

* It seems that approach needs the ground truth to train the pose-estimator. This is a major drawkback in my opinion. Having access to such information kind of undermines the whole endeavor. It is also not clear to me at all why the process of learning the pose-estimator is coupled with RL.

* RHP appears to be using the predictors learned via RL, value function, and pose-estimator. The paper mentions that these generally only return informative actions for a couple of time steps in a model-free setting. Why are they then used offline to do planning over a long horizon? I understand that planning in the space images is hard, but I don't see the motivation for not going completely model-free. Or at least I do not see why the planning performs well, while using quantaties approximated while doing RL. It is important for the authors to clarify this point.

* Has the experiment where the model-free approach is tested alone been tuned for best performance, or did the authors just adopt the best hyperparameters that worked for their approach and use them in the model-free scenario?

* Please add evaluations of sample complexity and learning behavior when comparing to model-free RL. It is not clear to me how many real samples one experiment/task has taken. I think this is a crucial indicator of applicability in a real scenario.

* A general question: Is there any sense in which this approach is actually solving a POMDP in the classical sense, i.e. is taking information-gathering actions? It would be interesting to highlight such behavior.


# Minor Comments:
---------------------------
* The paper refers to the proposed method as a "robust manipulation", that seems like a vague term. Can you expand on this?

* line 14: everyday-day

4. Was the video submission useful? What was good about it? What could be done to improve it? (Write N/A if there was no video submission)
The video is of very good quality.
5. If code was submitted, we ask that you perform a sanity check. We do not ask that you run the code. But if you do, please comment on this too. Authors have been instructed to provide a readme file that points to the part of the code that needs to be peer-reviewed. Please, read this part of the code and answer the following questions: a) Does the code appear to implement the algorithm described in the paper? b) Did the readme file allow you to identify relevant parts of the code? c) Were you provided with data to replicate the results? Please, remember that code is for peer-review only and that you are not allowed to use this code outside the review process. (Write N/A if there was no code submission)
N/A
9. Comment on the potential impact of the paper to real robotics problems (taking COVID-19 impact into account). Please check the supplement material for the COVID-19 response.
I think the problem the paper is tackling is important but I feel that the paper is missing too many details and leaves many open questions in general.

Also, the applicability in a real setting is not clear given some missing information about sample complexity and the need for a ready simulation of the environment.
12. Overall recommendation:
Weak Reject
13. Rate your level of confidence in this recommendation:
High
